Individual Rationality Conditions of Identifying Matching Costs in Transferable Utility Matching Games

As the widely applied method for measuring matching assortativeness in a transferable utility matching game, a matching maximum score estimation is proposed by \cite{fox2010qe}. This article reveals that combining unmatched agents, transfers, and individual rationality conditions with sufficiently large penalty terms makes it possible to identify the coefficient parameter of a single common constant, i.e., matching costs in the market.

==> 01intro.tex <==
\section{Introduction}
One of the most well-known methods for measuring matching assortativeness was developed by \cite{fox2010qe}. Although the method allows researchers to incorporate additional inequalities flexibly coming from equilibrium conditions, it is not known what additional information improves identification and estimation and to what extent. In this article, I focus on pairwise stability in a transferable utility (TU, henceforth) matching model and explore the practical improvement of identification and estimation by adding unmatched agents, transfer data, and individual rationality conditions.

Literature on measuring identification power is growing.\footnote{See recent survey such as \cite{aradillas2020econometrics}.} \cite{aradillas2008identification} examine the identification power of equilibrium in some simple strategic games. They investigate how the equilibrium assumptions shape identified sets. Recently, partial identification literature is one of the fastest growing area led by not only theoretical econometricians but also applied empirical economists.\footnote{See recent surveys such as \cite{molinari2020microeconometrics} and \cite{chesher2020generalized} for reference.} Thus, identification power improvement with a simple trick alleviates their practical concerns and increases the applicability of the structural model.

The literature on the empirical matching model is growing and closely related to the literature on partial identification.  \cite{uetake2013estimating} focus on a one-to-one non-transferable utility (NTU, henceforth) matching game allowing multiple equilibria and investigate the identification power by Monte Carlo simulation. \cite{echenique2013partial} also study both TU and NTU models by applying a moment inequality approach to repeated observations of matchings among a fixed group of individuals. \cite{fox2010qe} proposes a semiparametric model called as matching maximum score estimator in a TU matching game and reports Monte Carlo studies showing that the finite-sample performance of the matches-only maximum score estimator in many markets is good. \cite{fox2018qe} also shows that the matching maximum score estimator works for both point-identified and set-identified models with empirical applications in multiple markets setting. The approach has been used in many empirical applications.\footnote{Another popular approach is developed by \cite{galichon2021cupid}. As a recent survey, \cite{chiappori2016econometrics} provide a unified view of several empirical approaches in matching games.}

Following \cite{fox2010qe}, this article focuses on the matching maximum score estimator in a single market setting and provides unified and comparable computational results inspired by three practical devices to improve the identification power and estimation accuracy; (1) transfer data, (2) unmatched agents, and (3) individual rationality conditions. First, transfer data is known to improve identification power practically if it is available. The working paper version of \cite{fox2013aej} uses bidding price data in FCC Spectrum Auction in a single market setting. They numerically confirm that if the number of agents is small or the variance of errors is large, bidding price data generated from a tatonnement process drastically reduces the bias and RMSE (the root of mean squared error) of an estimated single parameter. \cite{akkus2015ms} use acquisition prices between buyer firms and target firms as transfer data. \cite{pan2017determinants} uses CEO compensations between CEOs and firms. Appendix A of \cite{akkus2015ms} shows Monte Carlo evidence that adding transfers not only improves the accuracy of estimation but also enables researchers to identify the coefficient of a non-interacted term. However, they did not show why adding the transfer data improve the identification power and estimation accuracy and not consider possibly negative assortativeness.

Second, there is some theoretical and empirical evidence that using unmatched agents helps identification. \cite{fox2018jpe} show nonparametric identification results in two-sided matching model. Section 5 of their paper proves that the distribution of unobserved complementarities conditional on observed characteristics can be recovered if each firm on each side is part of exactly one match or is unmatched in each feasible assignment. \cite{otani2021coalitional} uses unmatched firms to identify and estimate matching costs in a one-sided one-to-many coalitional mergers in Japanese shipping industry with Monte Carlo simulations. As far as I know, there is no computational work investigating the potential importance of unmatched agents to identification and estimation in the standard one-to-one two-sided matching model.

Third, individual rationality (IR, henceforth) conditions, i.e., the binary choice information are necessary for identification of a fixed cost \citep{bresnahan1990entry}. In the TU matching game, IR conditions capture whether agents choose to stay matched or unmatched. This article shows under what conditions matching fixed costs can be identified and estimated. 

This article finds that a combination of unmatched and transfer data gives the most accurate estimates. Second, IR conditions enable us to identify a coefficient of an additive separable constant such as matching fixed costs common in the market. Also, this paper finds that an additional importance weight of IR conditions is necessary for obtaining the lower bound of the matching fixed cost. 

The rest of the paper is organized as follows. Section \ref{sec:baseline_model} outlines the baseline model and how additional information work. Section \ref{sec:identification_of_matching_cost} investigates the identification of matching fixed costs. Section \ref{sec:simulation_bound} describes the Monte Carlo experiments and reports the results. Section \ref{sec:conclusion} discusses my findings and concludes, including practical suggestions. Appendix \ref{sec:supplemental_results} shows additional numerical checks.

% \begin{table}[]
%     \centering\scriptsize{}
%     \begin{tabular}{l|c}
%          & Paper \\\hline
%       transfer data used  & \cite{fox2013aej}, \cite{akkus2015ms}, \cite{pan2017determinants}, Amir et al?(2021) \\
%       unmatched data used & Xunjie?(2021), Otani? (2021)\\
%       transfer and unmatched data used & Kambayashi et al? (2021)\\
%     \end{tabular}
%     \caption{Literature}
%     \label{tb:literature_classification}
% \end{table}

==> 02model.tex <==
\section{Model}\label{sec:baseline_model}

\subsection{Baseline matching model}
Consider a two-sided one-to-one TU merger matching game. For simplicity, I consider a single matching market. Let $\mathcal{N}_b$ and $\mathcal{N}_s$ be the sets of potential finite buyers and sellers respectively. Let $b=1,\cdots,|\mathcal{N}_b|$ be individual buyer firms and $s=1,\cdots,|\mathcal{N}_s|$ be individual seller firms where $|\cdot|$ is cardinality. Let $\mathcal{N}_{b}^{m}$ be the set of ex-post matched buyers and $\mathcal{N}_{b}^{u}$ be that of ex-post unmatched buyers such that $\mathcal{N}_b= \mathcal{N}_{b}^{m}\cup\mathcal{N}_{b}^{u}$ and $\mathcal{N}_{b}^{m}\cap\mathcal{N}_{b}^{u}=\emptyset$. For the seller side, define $\mathcal{N}_{s}^{u}$ and $\mathcal{N}_{s}^{m}$ as the set of ex-post matched and unmatched sellers such that $\mathcal{N}_s= \mathcal{N}_{s}^{m}\cup\mathcal{N}_{s}^{u}$ and $\mathcal{N}_{s}^{m}\cap\mathcal{N}_{s}^{u}=\emptyset$. Let $\mathcal{M}^m$ be the sets of all ex-post matched pairs $(b,s)\in\mathcal{N}_{b}^{m}\times \mathcal{N}_{s}^{m}$. Also, let $\mathcal{M}$ be the set of all ex-post matched pairs $(b,s)\in\mathcal{M}^{m}$ and unmatched pairs $(\tilde{b},\emptyset)$ and $(\emptyset,\tilde{s})$ for all $\tilde{b}\in \mathcal{N}_b^u$ and $\tilde{s}\in \mathcal{N}_s^u$ where $\emptyset$ means a null agent generating unmatched payoff. 

Each firm can match at most one agent on the other side so that $|\mathcal{N}_b^{m}|=|\mathcal{N}_s^{m}|$. The post-merger real-valued matching joint production function is defined as $f(b,s)=V_b(b,s)+V_s(b,s)$. The net post-merger values for buyer $b$ and seller $s$ are also defined as $V_b(b,s)=f(b,s)-p_{b,s}$ and $V_s(b,s)+p_{b,s}$ where $p_{b,s}\in \mathbb{R}_{+}$ is equilibrium merger price paid to seller firm $s$ by buyer firm $b$ and $p_{b\emptyset}=p_{\emptyset s}=0$. For scale normalization, I assume the standard assumption that the value of unmatched is zero, i.e., $V_b(b,\emptyset)=0$ and $V_s(\emptyset,s)=0$ for all $b\in \mathcal{N}_b$ and $s\in \mathcal{N}_s$. Each buyer maximizes $V_b(b,s)$ across seller firms, whereas each seller maximizes $V_s(b,s)$ across buyer firms. 

The stability conditions for buyer firm $b \in \mathcal{N}_b$ and seller firm $s \in \mathcal{N}_s$ are written as:
\begin{align}
    V_b(b,s) &\ge V_b(b,s') \quad \forall s' \in \mathcal{N}_s \cup \emptyset,s'\neq s,\label{eq:stability_ineq}\\
    V_s(b,s) &\ge V_s(b',s) \quad \forall b' \in \mathcal{N}_b\cup \emptyset,b'\neq b.\nonumber
\end{align}
Buyer firm $b$ and seller firm $s$ can be either matched or unmatched one.

For constructing pairwise inequalities based on  equation \eqref{eq:stability_ineq}, I define the inequalities for matches $(b,s)\in \mathcal{M}$ and $(b',s')\in \mathcal{M}, (b',s')\neq(b,s)$ as:
\begin{align*}
    f(b,s)-p_{b,s}&\ge f(b,s')-p_{b,s'},\\
    f(b',s')-p_{b',s'}&\ge f(b',s)-p_{b',s},\\
    V_s(b,s)+p_{b,s}&\ge V_s(b',s)+p_{b',s},\\
    V_{s'}(b',s')+p_{b',s'}&\ge V_s(b,s')+p_{b,s'},
\end{align*}
where $p_{b',s}$ and $p_{b,s'}$ are unrealized equilibrium merger prices which cannot be observed in the data. \cite{akkus2015ms} show that equilibrium transfer $p_{b,s'}$ from a competing buyer $b$ to seller $s'$ must be weakly smaller than the offer $p_{b's'}$ from matched buyer $b'$. This means that seller firm obtains a weakly higher transfer from a matched pair than the other unmatched pairs. Thus, by substituting $p_{b',s}\le p_{b,s}$ and $p_{b,s'}\le p_{b',s'}$, I finally obtain the following inequalities for matches $(b,s)$ and $(b',s')$:
\begin{align}
    f(b,s)-f(b,s')&\ge p_{b,s}-p_{b,s'}\ge p_{b,s}-p_{b',s'},\label{eq:pairwise_stable_ineq}\\
    f(b',s')-f(b',s)&\ge p_{b',s'}-p_{b',s}\ge p_{b',s'}-p_{b,s},\nonumber\\
    V_s(b,s)-V_s(b',s)&\ge 0,\nonumber\\
    V_{s'}(b',s')-V_s(b,s')&\ge 0,\nonumber
\end{align}
where the last two inequalities cannot be available from the data because researchers cannot observe how the total matching value $f(b,s)$ is shared between buyer $b$ and seller $s$.





% \subsection{Unmatched agents}\label{subsec:unmatched}

% With no additional assumptions, I construct additional inequalities for unmatched firm $u\in\mathcal{N}_s^{u}$ on the buyer side and unmatched firm $v\in\mathcal{N}_s^{u}$ on the seller side as:
% \begin{align}
%     0=V_b(u,\emptyset) &\ge V_b(u,v')=f(u,v')-p_{uv'} \quad \forall v' \in \mathcal{N}_s^{u}\label{eq:unmatched_ineq}\\
%     0=V_s(\emptyset,v) &\ge V_s(u',v)=f(u',v)-p_{u'v} \quad \forall u' \in \mathcal{N}_b^{u},\nonumber
% \end{align}
% where the second inequality cannot be available from the data analogously. \textcolor{blue}{The equilibrium price condition allows us to substitute $p_{uv'}=0$.} Note that equation \eqref{eq:unmatched_ineq} is a strict subset of equation \eqref{eq:stability_ineq}. However, if the researchers ignore the existence of unmatched firms, then equation \eqref{eq:unmatched_ineq} which provides informative inequalities cannot be constructed.


\subsection{Transfer and unmatched data.}

In many empirical applications, researchers do not obtain data about transfers and unmatched firms. Based on inequalities \eqref{eq:pairwise_stable_ineq}, I formally state the minimum number of possible inequalities, which is dependent on data availability.
\begin{proposition}\label{prop:num_of_all_ineq}
    Suppose that researchers obtain one-to-one two-sided matching data which contains observed characteristics of all matched buyers in $\mathcal{N}^m_b$ and sellers in $\mathcal{N}^m_s$, (1) transfer data $p_{bs}$ for matched buyer firm $b$ and seller firm $s$ for all $b\in\mathcal{N}_b^{m}$ and $s\in\mathcal{N}_s^{m}$, and (2) unmatched data about $\mathcal{N}_b^{u}$ and $\mathcal{N}_s^{u}$ with their observed characteristics. Let $_nC_k$ be the number of combinations of $k$ objects from $n$ objects, and $_nP_k$ be the number of permutations which count the different ordered arrangements of a $k$-element subset of a $n$-set.\footnote{For reference, $_nC_k=\frac{n!}{k!(n-k)!}$ and $_nP_k=\frac{n!}{(n-k)!}$ where $!$ is a factorial function.} Then, 
    \begin{enumerate}
        \renewcommand{\labelenumi}{(\roman{enumi})}
        \item the researchers can construct the following inequalities: for matches $(b,s)\in \mathcal{M}$ and $(b',s')\in \mathcal{M}, (b',s')\neq(b,s)$,
        \begin{align}
            f(b,s)-f(b,s')&\ge p_{b,s}-p_{b',s'}.\label{eq:inequality_with_transfer}
        \end{align}
        Also, the minimum number of total inequalities is $_{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}P_2$.
        \item If the data does not contain (1), the researchers can construct the following inequalities: for matches $(b,s)\in \mathcal{M}$ and $(b',s')\in \mathcal{M}, (b',s')\neq(b,s)$,
        \begin{align}
            f(b,s)+ f(b',s')&\ge f(b,s')+f(b',s).\label{eq:inequality_without_transfer}
        \end{align}
        Also, the minimum number of total inequalities is $_{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}C_2$.
        \item If the data does not contain (2), the researchers can construct inequality \eqref{eq:inequality_without_transfer} for matches $(b,s)\in \mathcal{M}^m$ and $(b',s')\in \mathcal{M}^m, (b',s')\neq(b,s)$. Also, the minimum number of total inequalities is $_{|\mathcal{M}^m|}P_2$.
        \item If the data does not contain (1) and (2), the researchers can construct inequality \eqref{eq:inequality_with_transfer} for matches $(b,s)\in \mathcal{M}^m$ and $(b',s')\in \mathcal{M}^m, (b',s')\neq(b,s)$. Also, the minimum number of total inequalities is $_{|\mathcal{M}^m|}C_2$.
    \end{enumerate}
\end{proposition}
\begin{proof}
For proving $(i)$, note that $\mathcal{M}$ restores unmatched buyer $\tilde{b}$ and seller $\tilde{s}$ as $(\tilde{b},\emptyset)$ and $(\emptyset,\tilde{s})$ so that the size of the set of unmatched pairs is $(|\mathcal{N}_b^u|+|\mathcal{N}_s^u|)$.
Thus, the number of possible combinations of $(b,s)\in \mathcal{M}$ and $(b',s')\in \mathcal{M}, (b',s')\neq(b,s)$ is $_{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}C_2$ and each combination gives two inequalities as in inequality \eqref{eq:inequality_with_transfer}. This gives $$
2\cdot _{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}C_2=2\frac{(|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|)(|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|-1)}{2!}=_{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}P_2,
$$
by definitions of $C$ and $P$.

For proving $(ii)$, the number of possible combinations of $(b,s)\in \mathcal{M}$ and $(b',s')\in \mathcal{M}, (b',s')\neq(b,s)$ is the same as $(i)$ but each combination gives a single inequality as in inequality \eqref{eq:inequality_without_transfer}. For proving $(iii)$ and $(iv)$, substituting $|\mathcal{N}_s^u| = |\mathcal{N}_b^u|=0$ into $(i)$ and $(ii)$ gives the results. 
\end{proof}

Note that it is possible to add inequalities by using research-specific institutional details such as a subsidy and deregulation. Proposition \ref{prop:num_of_all_ineq} not only gives quite simple results about the minimum number of pairwise inequalities but also illustrates a useful decomposition of pairwise inequalities, which is used in Proposition \ref{prop:identification_of_matching_cost}.


\subsection{Individual rationality conditions}

The individual rationality (IR) conditions are included implicitly in inequality \eqref{eq:inequality_with_transfer} when transfer data is available because $\mathcal{M}$ restores unmatched buyer $\tilde{b}$ and seller $\tilde{s}$ as $(\tilde{b},\emptyset)$ and $(\emptyset,\tilde{s})$. For matched pair $(b,s)\in \mathcal{M}$ and unmatched buyer $(\tilde{b},\emptyset)\in \mathcal{M}$, inequality \eqref{eq:inequality_with_transfer} gives $f(b,s)-f(b,\emptyset)=f(b,s)\ge p_{b,s}-p_{\tilde{b},\emptyset}\ge p_{b,s}$, i.e., 
\begin{align}
    f(b,s)-p_{b,s}&\ge 0. \label{eq:IR_condition} 
\end{align}
Importantly, unlike pairwise inequalities, the IR condition holds for each matched firm on each side regardless of the availability of transfer data. To distinguish IR conditions from pairwise inequalities, let $IR(\mathcal{M}^m)=2|\mathcal{M}^m|=|\mathcal{M}_b^m|+|\mathcal{M}_s^m|$ be the number of inequalities from IR conditions.

Table \ref{tb:num_inequalities} summarizes the above results. Note that $_{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}P_2$ and $_{|\mathcal{M}^m|}P_2$ include the same inequalities in $IR(\mathcal{M}^m)$. Proposition \ref{prop:num_of_all_ineq} does not show, however, how the existence of unmatched firms, transfer data, and IR conditions contributes to identification and matching maximum score estimation. In Section \ref{sec:identification_of_matching_cost}, I show a trivial but necessary modification for identification and estimation of matching costs.

\begin{table}[!ht]
\caption{\textbf{The minimum number of total inequalities.}}
\centering
\begin{tabular}{cc|c|c| } 
 \hline
 &&\multicolumn{2}{|c|}{unmatched} \\
 && available & unavailable \\ 
 \hline
 transfer&available & $_{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}P_2$ & $_{|\mathcal{M}^m|}P_2$ \\ \hline
 &unavailable & $_{|\mathcal{M}^m|+|\mathcal{N}_b^u|+|\mathcal{N}_s^u|}C_2+IR(\mathcal{M}^m)$ & $_{|\mathcal{M}^m|}C_2+IR(\mathcal{M}^m)$ \\ 
 \hline
\end{tabular}
\label{tb:num_inequalities}
\end{table}


\subsection{Matching Maximum Score Estimator}\label{subsec:matching_maximum_score_estimator}

\cite{fox2010qe} proposes maximum score
estimator that makes use of inequalities introduced in inequality \eqref{eq:inequality_with_transfer} or inequality \eqref{eq:inequality_without_transfer}. The maximum score estimator is consistent if the model satisfies a rank order property, i.e., the probability of observing matched pairs is larger than the probability of observing swapped matched pairs.\footnote{See \cite{fox2010qe} and \cite{fox2018qe} for theoretical conditions and results.} I specify $f(b,s)$ as a parametric form $f(b,s|X,\beta)$ where $X$ is a vector of observed characteristics of all buyers and sellers. Given observed characteristics $X$, one can estimate the parameter vector $\beta$ without IR conditions by maximizing the following objective function:
\begin{align}
    Q(\beta)=\begin{cases}
         \sum_{(b,s)\in \mathcal{M}} \sum_{(b',s')\in \mathcal{M},(b',s')\neq (b,s)} \mathbbm{1}[f(b,s|X,\beta)-f(b,s'|X,\beta)\ge p_{b,s}-p_{b',s'}]\\
         \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \text{if transfer data is available},\\
         \sum_{(b,s)\in \mathcal{M}} \sum_{(b',s')\in \mathcal{M},(b',s')\neq (b,s)} \mathbbm{1}[f(b,s|X,\beta)+ f(b',s'|X,\beta)\ge f(b,s'|X,\beta)+f(b',s|X,\beta)]\\
         \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \text{otherwise},
    \end{cases}\label{eq:score_function}
\end{align}
where $\mathbbm{1}[\cdot]$ is an indicator function. If unmatched data is unavailable, $\mathcal{M}$ is replaced by $\mathcal{M}^m$. 
Concretely, $Q(\beta)$ is the number of times the inequality in the right-hand side is satisfied given the candidate parameter $\beta$. 
If IR conditions are included, the objective function $Q(\beta)$ is modified into
\begin{align}
    \tilde{Q}(\beta)=Q(\beta) + \lambda\cdot\sum_{(b,s)\in \mathcal{M}^m}  1[f(b,s|X,\beta)\ge 0], \quad \lambda \ge 1,\label{eq:score_function_with_IR}
\end{align}
where let $\lambda$ be called the importance weight of IR conditions. If $\lambda$ is larger, the importance of IR condition term is larger for the evaluation of $\tilde{Q}(\beta)$. If transfer data is available, the correction term is redundant as shown in Table \ref{tb:num_inequalities}, but it does not affect searching the maximizer of $\tilde{Q}(\beta)$. Section \ref{sec:identification_of_matching_cost} investigates the importance of $\lambda$.

Since indicator functions exist in the objective function \eqref{eq:score_function} and \eqref{eq:score_function_with_IR}, $Q(\beta)$ and $\tilde{Q}(\beta)$ are not differentiable. To find maximizers of $Q(\beta)$ and $\tilde{Q}(\beta)$, I use Differential Evolution algorithm developed by \cite{storn1997differential}.







% \subsection{The improvement of identification power with unmatched firms and transfer data.}\label{subsec:supplement_identification_region_plot}
% \input{02supplement_identification_region_plot}





==> 02supplement_identification_region_plot.tex <==
The parameter $\beta$ is estimated as a maximizer or a set of maximizers of $Q(\beta)$ or $\tilde{Q}(\beta)$ so that $\beta$ lie within a high-dimensional polytope determined by inequalities in Table \ref{tb:num_inequalities}. Although it is difficult to show the general case, I show what type of inequality corresponds with a hyperplane restricting identified set of $\beta$ in Section \ref{subsec:supplement_identification_region_plot}.

To illustrate the restriction power of inequalities, I introduce a simple example. Let $\mathcal{M}_{b}^m=\{1,2\}$, $\mathcal{M}_{b}^u=\{3\}$, $\mathcal{M}_{s}^m=\{a,b\}$, and $\mathcal{M}_{s}^u=\{c\}$. Suppose that I observe matched pairs $(1,a)$ and $(2,b)$ and unmatched pairs $(3,\emptyset)$ and $(\emptyset,c)$. I specify the total matching value $f(b,s)=1\cdot \bar{X}_{b,s}+X_{b,s}\beta$ where $1$ is a normalized constant parameter, $\beta\in\mathbb{R}$, two dimensional match-specific observed characteristic $(\bar{X}_{b,s},X_{b,s})\in\mathbb{R}\times \mathbb{R}$, and $p_{b,s}$ is a transfer for matches $(b,s)$. When transfer data is available, by Table \ref{tb:num_inequalities}, reserachers can construct $_4C_3=12$ inequalities. Our objective is to find the set of $\beta$ which satisfies all inequalities summarized as:
\begin{align}
    \begin{cases}
         f(1, a)-f(1, b) \geq p_{1 a}-p_{1 b} \\
f(1, a)-f(1, c) \geq p_{1 a}-p_{1 c} \\
f(1, a)-f(1, \emptyset) \geq p_{1 a}-p_{1\emptyset} \\
f(2, b)-f(2, a) \geq p_{2 b}-p_{2 a} \\
f(2, b)-f(2, c) \geq p_{2 b}-p_{2 c} \\
f(2, b)-f(2, \emptyset) \geq p_{2 b}-p_{2\emptyset} \\
f(3, \emptyset)-f(3, a) \geq p_{3 \emptyset}-p_{3 a} \\
f(3, \emptyset)-f(3, b) \geq p_{3\emptyset}-p_{3 b} \\
f(3, \emptyset)-f(3, c) \geq p_{3 \emptyset}-p_{3 c}\\
f(\emptyset, c)-f(1, c) \geq p_{\emptyset,c}-p_{1 c} \\
f(\emptyset, c)-f(2, c) \geq p_{\emptyset,c}-p_{2 c} \\
f(\emptyset, c)-f(3, c) \geq p_{\emptyset,c}-p_{3 c}
    \end{cases}
\rightarrow \begin{cases}
    (\bar{X}_{1a}-\bar{X}_{1b})+(X_{1a}-X_{1b})\beta \ge p_{1a}-p_{2b}\\
    (\bar{X}_{1a}-\bar{X}_{1c})+(X_{1a}-X_{1c})\beta \ge p_{1a}-p_{1c}\\
    \bar{X}_{1a}+X_{1a}\beta \ge p_{1a}\\
    (\bar{X}_{2b}-\bar{X}_{2a})+(X_{2b}-X_{2a})\beta \ge p_{2b}-p_{1a}\\
    (\bar{X}_{2b}-\bar{X}_{2c})+(X_{2b}-X_{2c})\beta \ge p_{2b}-p_{2c}\\
    \bar{X}_{2b}+X_{2b}\beta \ge p_{2b}\\
    \bar{X}_{3a}+X_{3a}\beta \le p_{3a}\le p_{1a}\\
    \bar{X}_{3b}+X_{3b}\beta \le p_{3b}\le p_{2b}\\
    \bar{X}_{3c}+X_{3c}\beta \le p_{3c}= 0 \\
    \bar{X}_{1c}+X_{1c}\beta \le p_{1c}\\
    \bar{X}_{2c}+X_{2c}\beta \le p_{2c}\\
    \bar{X}_{3c}+X_{3c}\beta \le p_{3c}= 0 
\end{cases},\label{eq:example_all_ineq}
\end{align}
where I substitute $p_{2b}\ge p_{1b}$, $p_{1a}\ge p_{2a}$, and $p_{3c}= 0$ under the equilibrium price property as in \cite{akkus2015ms}.

Suppose that the researchers do not have data about transfers but unmatched firms. Then, by Table \ref{tb:num_inequalities}, they can construct $\frac{1}{2}\cdot 4 \cdot 3=6$ inequalities as: 

\begin{align}
    \begin{cases}
f(1, a) + f(2, b) \geq f(1, b)+f(2, a) \\
f(1, a) + f(3, \emptyset) \geq f(1,\emptyset) + f(3, a)\\
f(2, b) + f(3, \emptyset) \geq f(2, \emptyset) + f(3, b)\\
f(1, a) + f(\emptyset, c) \geq f(1, c)+f(\emptyset, a) \\
f(2, b) + f(\emptyset, c) \geq f(2, c) + f(\emptyset, b)\\
f(3, \emptyset) + f(\emptyset, c) \geq f(3, c) + f(\emptyset, \emptyset)
\end{cases}\rightarrow \begin{cases}
    (\bar{X}_{1a}+\bar{X}_{2b}-\bar{X}_{1b}-\bar{X}_{2a})+(X_{1a}+X_{2b}-X_{1b}-X_{2a})\beta \ge 0\\
    (\bar{X}_{1a}-\bar{X}_{3a})+(X_{1a}-X_{3a})\beta \ge 0\\
    (\bar{X}_{2b}-\bar{X}_{3b})+(X_{2b}-X_{3b})\beta \ge 0\\
    (\bar{X}_{1a}-\bar{X}_{1c})+(X_{1a}-X_{1c})\beta \ge 0\\
    (\bar{X}_{2b}-\bar{X}_{2c})+(X_{2b}-X_{2c})\beta \ge 0\\
    0 \ge \bar{X}_{3c}+X_{3c}\beta.
\end{cases}\label{eq:num_ineq_without_transfer}
\end{align}

Suppose that the researchers do not have data about unmatched firms but transfers. Then, by Table \eqref{tb:num_inequalities}, they can construct $2$ inequalities as: 
\begin{align}
    \begin{cases}
f(1, a)-f(1, b) \geq p_{1 a}-p_{1 b} \\
f(2, b)-f(2, a) \geq p_{2 b}-p_{2 a} 
\end{cases}\rightarrow \begin{cases}
    (\bar{X}_{1a}-\bar{X}_{1b})+(X_{1a}-X_{1b})\beta \ge p_{1a}-p_{2b}\\
    (\bar{X}_{2b}-\bar{X}_{2a})+(X_{2b}-X_{2a})\beta \ge p_{2b}-p_{1a}.
\end{cases}\label{eq:num_ineq_without_unmatched}
\end{align}

Suppose that the researchers do not have data about transfers and unmatched firms. Then, by Table \eqref{tb:num_inequalities}, they can construct $1$ inequality as: 
\begin{align}
    &\begin{array}{l}
f(1, a) + f(2, b) \geq f(1, b)+f(2, a) 
\end{array}\nonumber\\
     &\rightarrow \begin{array}{l}
    (\bar{X}_{1a}+\bar{X}_{2b}-\bar{X}_{1b}-\bar{X}_{2a})+(X_{1a}+X_{2b}-X_{1b}-X_{2a})\beta \ge 0.
\end{array}\label{eq:num_ineq_without_transfer_and_unmatched}
\end{align}

Note that the set of inequalities \eqref{eq:num_ineq_without_unmatched} is a strict subset of inequalities \eqref{eq:example_all_ineq} and the set of the inequalities \eqref{eq:num_ineq_without_transfer_and_unmatched} is a strict subset of inequalities \eqref{eq:num_ineq_without_transfer}. Thus, monotonicity of the sets of equilibrium constraints indicates that the identification power decreases as \eqref{eq:example_all_ineq} is replaced with \eqref{eq:num_ineq_without_unmatched} and \eqref{eq:num_ineq_without_transfer} is replaced with \eqref{eq:num_ineq_without_transfer_and_unmatched}. Thus, I only need to show that the identification power decreases as inequalities \eqref{eq:example_all_ineq} is replaced with inequalities \eqref{eq:num_ineq_without_transfer}. Formally, I need to compare
\begin{align*}
    \begin{array}{l}
    \begin{cases}
         (\bar{X}_{1a}-\bar{X}_{1b})+(X_{1a}-X_{1b})\beta \ge p_{1a}-p_{2b}\\
         (\bar{X}_{2b}-\bar{X}_{2a})+(X_{2b}-X_{2a})\beta \ge p_{2b}-p_{1a}
    \end{cases}
\end{array}\text{and}\quad
\begin{array}{l}
    (\bar{X}_{1a}+\bar{X}_{2b}-\bar{X}_{1b}-\bar{X}_{2a})\\
    \quad\quad\quad+(X_{1a}+X_{2b}-X_{1b}-X_{2a})\beta \ge 0,
\end{array}
\end{align*}
since the other inequalities in \eqref{eq:example_all_ineq} are analogously derived. Let the comparison be denoted concisely as:
\begin{align*}
    \begin{array}{l}
    \begin{cases}
         A+B\beta \ge C\\
         D+E\beta \ge -C
    \end{cases}
\end{array}\text{and}\quad (A+D)+(B+E)\beta \ge 0.
\end{align*}
Without of loss generality, assume $C>0$. Then, the inequalities are expressed as
\begin{align}
    \begin{array}{l}
    \begin{cases}
         \beta \ge \frac{C-A}{B}\\
         \frac{C+D}{-E} \ge \beta
    \end{cases}
\end{array}\text{and}\quad \beta \ge \frac{-(A+D)}{(B+E)}.\label{eq:ineq_concise}
\end{align}
Whenever $\frac{C+D}{-E}\ge \frac{C-A}{B}$ or $\frac{C+D}{-E}\le \frac{C-A}{B}$, the left equations can be bounded by the two composite terms.

To illustrate the power of inequality restrictions for each inequality, I fix some elements determined by data. Assume that $C=1$ and $A=D=0$, i.e., the first observed characteristic has no effect on the inequalities. Then, \eqref{eq:ineq_concise} is reduced to
\begin{align*}
    \begin{array}{l}
    \begin{cases}
         \beta \ge \frac{1}{B}\\
         \frac{1}{-E} \ge \beta
    \end{cases}
\end{array}\text{and}\quad (B+E)\beta \ge 0.
\end{align*}
I denote the left equations as \textit{separated inequalities} and the right equation as \textit{composite inequality}. Also, I denote $\beta \le \frac{-\bar{X}_{3c}}{X_{3c}}$ derived from the ninth line of inequalities \eqref{eq:example_all_ineq} as \textit{unmatched inequality} and fix constant $\frac{-\bar{X}_{3c}}{X_{3c}}=5$.

Figure \ref{fg:identification_region_3d} illustrates the upper and lower bounds of $\beta$ induced by separated inequalities (red and blue), lower bound of $\beta$ induced by composite inequality (green), and upper bound of the unmatched inequality (yellow). Note that the $\beta$ in the composite inequality is upper unbounded for each matching pair. The figure focuses only on the domains (the case of $B>0, E>0$ and the case of $B>0, E<0$), however, the other domains can be analogously illustrated. First, I find that the identification power decreases when inequalities \eqref{eq:example_all_ineq} is reduced to inequalities \eqref{eq:num_ineq_without_transfer} because the identification set derived from the composite inequality is much larger than the identification set derived from the separated inequalities. Second, the identification set shrinks as $B$ and $E$ is larger. This means that the differences of match-specific characteristics between the observed match and swapped match help identification of $\beta$ significantly. Third, unmatched inequality help identification significantly especially when $B$ and $E$ are close to zero, i.e., the differences of match-specific characteristics between the observed match and swapped match are small.

In the above simple example, I find how each type of inequality in each matching pair characterizes the identified set of $\beta$. In the general model, the identified set is characterized as a polytope. In Section \ref{sec:simulation_bound}, I investigate how each type of inequality contributes to the identification totally through the objective function of the matching maximum score estimator.

\begin{figure}[htbp]
  \begin{minipage}{0.5\hsize}
  \begin{center}
   \includegraphics[width=60mm]{figuretable/identification_region_3d_positive_B_positive_E.png}
  \end{center}
 \end{minipage}
 \begin{minipage}{0.5\hsize}
  \begin{center}
   \includegraphics[width=60mm]{figuretable/identification_region_3d_positive_B_negative_E.png}
  \end{center}
 \end{minipage}
 \caption{\textbf{The identification power of inequalities for each matching pair}. Fix $C=1$ and $A=D=0$. The domains of left and right panels are restricted to ($B>0,E>0$) and ($B>0,E<0$) respectively. The red and blue surfaces mean the upper and lower bounds of parameter $\beta$ derived from the separated inequality in inequalities \eqref{eq:ineq_concise}. The roles of bounds are reversed in some domains in the right panel. The green surface means the lower (or upper) bounds of parameter $\beta$ derived from the composite inequality in inequalities \eqref{eq:ineq_concise}. The yellow surface means the upper bound of parameter $\beta$ derived from unmatched inequality and fixed to $5$.}
\label{fg:identification_region_3d}
\end{figure}

==> 03identification_of_matching_cost.tex <==
\section{IR conditions identify the coefficient parameter of a constant}\label{sec:identification_of_matching_cost}

The estimation of fixed costs is one of the fundamental tasks in structural empirical studies. Suppose that researchers want to estimate an additive separable matching cost in a single market. Let $c$ be the matching cost and assume $c<0$ for exposition.\footnote{If researchers expect $\beta X_bX_s$ to be negative, i.e., the market to generate negative assortative matchings and want to investigate a subsidy effect inducing matchings, they can assume $c>0$ as the subsidy effect. The logic is the same in the main text.} Following the literature, I specify $f(b,s)$ as follows:
\begin{align}
    f(b,s) = \beta X_b X_s + c \cdot\mathbbm{1}[b\neq \emptyset \text{ or } s\neq \emptyset],\label{eq:with_matching_cost}
\end{align}
where $X_b$ and $X_s$ are vectors of continuous observable characteristics for buyer $b$ and seller $s$ and $\beta$ is a vector of parameters. Note that hypothetical matching cost $c$ exists for unmatched pairs. Then, Proposition \ref{prop:identification_of_matching_cost} holds. 

\begin{proposition}\label{prop:identification_of_matching_cost}
Suppose the matching joint production function is specified as \eqref{eq:with_matching_cost}. Then,
\begin{enumerate}
    \renewcommand{\labelenumi}{(\roman{enumi})}
    \item by using pairwise inequalities based only on matched pairs, $c$ cannot be identified via $Q(\cdot)$;
    \item in addition to (i), even if transfer data is available, $c$ cannot be identified via $Q(\cdot)$;
    \item in addition to (i), even if unmatched data is available, the lower bound of $c$ cannot be identified without IR conditions;
    \item in addition to (iii), $c$ can be identified only when IR conditions are used with a sufficiently large importance weight via $\tilde{Q}(\beta)$, whether the transfer data is included or not. 
\end{enumerate}
\end{proposition}
\begin{proof}
To prove $(i)$, substituting \eqref{eq:with_matching_cost} into \eqref{eq:inequality_with_transfer} gives
\begin{align*}
    &\beta X_b X_s + c \cdot\mathbbm{1}[b\neq \emptyset \text{ or } s\neq \emptyset] + \beta X_{b'} X_{s'} + c \cdot\mathbbm{1}[b'\neq \emptyset \text{ or } s'\neq \emptyset]\\
    &\quad\ge \beta X_b X_{s'} + c \cdot\mathbbm{1}[b\neq \emptyset \text{ or } s'\neq \emptyset] + \beta X_{b'} X_s + c \cdot\mathbbm{1}[b'\neq \emptyset \text{ or } s\neq \emptyset],
\end{align*}
where the indicator functions must be 1 for matched pair $(b,s)$ and unrealized matched pair $(b,s')$ so that matching cost $c$ is canceled out. Similarly, $(ii)$ is also proved in the same way.

To prove $(iii)$, it is sufficient to consider pairwise inequalities based on an unmatched pair as the pairwise inequalities of matched pairs are shown above. With transfer data, by substituting \eqref{eq:with_matching_cost} into \eqref{eq:inequality_with_transfer}, the pairwise inequalities based on unmatched pairs denoted by $(\tilde{b},\emptyset)$ and $(\emptyset,\tilde{s})$ can be reduced to a single inequality as follows:
\begin{align*}
    0&\ge \beta X_{\tilde{b}} X_{\tilde{s}} + c - p_{\tilde{b},\tilde{s}},
\end{align*}
where $p_{\tilde{b},\tilde{s}}=0$. This only provides the upper bound of $c$ as $-\beta X_b X_s\ge c$. Without transfer data, the same inequality is derived using \eqref{eq:inequality_without_transfer}.

To prove $(iv)$, when transfer data is available, IR condition \eqref{eq:IR_condition} for matched pair $(b,s)$ gives
\begin{align*}
    \beta X_b X_s + c - p_{b,s}\ge 0,
\end{align*}
whereas, when transfer data is not available, IR condition \eqref{eq:IR_condition} for matched pair $(b,s)$ gives
\begin{align*}
    \beta X_b X_s + c \ge 0.
\end{align*}
Thus, IR condition \eqref{eq:IR_condition} provides the lower bound of $c$ as $c\ge -\beta X_b X_s+p_{b,s}$ or $c\ge -\beta X_b X_s$. 

Finally, I demonstrate the necessity of $\lambda$. In the modified objective function in \eqref{eq:score_function_with_IR}, the additional term
\begin{align*}
    \lambda\cdot\sum_{(b,s)\in \mathcal{M}^m}  1[\beta X_b X_s + c\ge 0],
\end{align*}
takes up to $\lambda\cdot |\mathcal{M}^m|$. However, $Q(\beta)$ of \eqref{eq:score_function_with_IR} can take up to either of the numbers in Table \ref{tb:num_inequalities} which are much larger than $|\mathcal{M}^m|$. In finite samples, the part does not need to achieve its perfect score, so some fractions of pairwise inequalities are not satisfied even at the maximizer of the objective function. This implies that, if $\lambda$ and $|\mathcal{M}^m|$ are small, the evaluation of IR conditions is dominated by the number of unsatisfied pairwise inequalities, which can be larger than $|\mathcal{M}^m|$. Thus, $\lambda$ must be large enough, corresponding to $|\mathcal{M}^m|$.
\end{proof}

Note that $(iv)$ of Proposition \ref{prop:identification_of_matching_cost} does not reveal how large the importance weight $\lambda$ should be. The appropriate weight of $\lambda$ depends on the sample sizes of matched and unmatched agents as a tuning parameter.








==> figuretable/estimation_results_single_market_two_param_beta1_with_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.39 & 0.33 & 0.17 & 0.03 & -0.0 \\
 &  & RMSE & (1.54) & (0.89) & (0.5) & (0.27) & (0.17) \\
 & T & Bias & 0.44 & 0.34 & 0.17 & 0.03 & -0.0 \\
 &  & RMSE & (1.61) & (0.89) & (0.5) & (0.27) & (0.17) \\
 & U & Bias & 0.47 & 0.34 & 0.16 & 0.03 & -0.0 \\
 &  & RMSE & (1.65) & (0.89) & (0.5) & (0.27) & (0.17) \\
 & Non & Bias & 0.43 & 0.34 & 0.16 & 0.03 & -0.0 \\
 &  & RMSE & (1.58) & (0.89) & (0.5) & (0.27) & (0.17) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.27 & 0.39 & 0.16 & 0.03 & -0.0 \\
 &  & RMSE & (1.38) & (0.99) & (0.5) & (0.27) & (0.17) \\
 & T & Bias & 0.23 & 0.4 & 0.16 & 0.03 & -0.0 \\
 &  & RMSE & (1.33) & (1.0) & (0.5) & (0.27) & (0.17) \\
 & U & Bias & 0.23 & 0.4 & 0.16 & 0.03 & -0.01 \\
 &  & RMSE & (1.33) & (1.0) & (0.5) & (0.27) & (0.17) \\
 & Non & Bias & 0.23 & 0.39 & 0.16 & 0.03 & -0.01 \\
 &  & RMSE & (1.33) & (0.99) & (0.5) & (0.27) & (0.17) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 2.44 & 4.77 & 6.51 & 10.48 & 19.2 \\
 & U,T & Bias & 0.89 & 0.46 & 0.23 & 0.2 & 0.14 \\
 &  & RMSE & (1.98) & (1.05) & (0.58) & (0.44) & (0.4) \\
 & T & Bias & 0.67 & 0.5 & 0.31 & 0.25 & 0.28 \\
 &  & RMSE & (1.46) & (1.14) & (0.57) & (0.49) & (0.5) \\
 & U & Bias & 0.89 & 0.48 & 0.26 & 0.22 & 0.16 \\
 &  & RMSE & (1.93) & (1.06) & (0.59) & (0.46) & (0.42) \\
 & Non & Bias & 0.67 & 0.5 & 0.31 & 0.26 & 0.29 \\
 &  & RMSE & (1.46) & (1.14) & (0.57) & (0.49) & (0.51) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.56 & 14.89 & 21.98 & 35.88 & 71.27 \\
 & U,T & Bias & 0.65 & 1.33 & 1.48 & 0.87 & 0.39 \\
 &  & RMSE & (3.08) & (3.26) & (3.27) & (2.24) & (1.09) \\
 & T & Bias & 0.81 & 0.63 & 0.43 & 0.45 & 0.41 \\
 &  & RMSE & (1.57) & (1.16) & (0.7) & (0.69) & (0.64) \\
 & U & Bias & 0.89 & 1.47 & 1.57 & 1.0 & 0.4 \\
 &  & RMSE & (3.29) & (3.44) & (3.36) & (2.37) & (1.09) \\
 & Non & Bias & 0.79 & 0.62 & 0.43 & 0.45 & 0.4 \\
 &  & RMSE & (1.55) & (1.14) & (0.7) & (0.69) & (0.63) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 9.77 & 19.47 & 28.86 & 47.81 & 95.1 \\
 & U,T & Bias & -0.66 & 0.87 & 1.66 & 2.45 & 2.1 \\
 &  & RMSE & (5.17) & (5.74) & (4.94) & (4.56) & (3.99) \\
 & T & Bias & -2.56 & -1.92 & -0.73 & 0.23 & 0.3 \\
 &  & RMSE & (4.48) & (4.16) & (3.16) & (1.44) & (0.61) \\
 & U & Bias & -0.71 & 0.83 & 1.59 & 2.44 & 2.32 \\
 &  & RMSE & (5.18) & (5.74) & (4.92) & (4.56) & (4.19) \\
 & Non & Bias & -2.56 & -1.92 & -0.75 & 0.22 & 0.31 \\
 &  & RMSE & (4.48) & (4.16) & (3.15) & (1.44) & (0.6) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta1_with_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.45 & 0.28 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (1.88) & (0.77) & (0.47) & (0.29) & (0.16) \\
 & T & Bias & 0.45 & 0.27 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (1.88) & (0.77) & (0.47) & (0.29) & (0.16) \\
 & U & Bias & 0.55 & 0.28 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (2.0) & (0.77) & (0.47) & (0.29) & (0.16) \\
 & Non & Bias & 0.46 & 0.28 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (1.88) & (0.77) & (0.47) & (0.29) & (0.16) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.5 & 0.32 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (1.96) & (0.9) & (0.47) & (0.29) & (0.16) \\
 & T & Bias & 0.54 & 0.32 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (1.99) & (0.9) & (0.47) & (0.29) & (0.16) \\
 & U & Bias & 0.54 & 0.32 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (1.99) & (0.9) & (0.47) & (0.29) & (0.16) \\
 & Non & Bias & 0.5 & 0.32 & 0.14 & 0.04 & 0.0 \\
 &  & RMSE & (1.96) & (0.9) & (0.47) & (0.29) & (0.16) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 2.59 & 4.68 & 6.33 & 10.27 & 18.64 \\
 & U,T & Bias & 0.84 & 0.29 & 0.07 & 0.05 & 0.01 \\
 &  & RMSE & (2.01) & (0.85) & (0.44) & (0.28) & (0.18) \\
 & T & Bias & 0.51 & 0.25 & 0.05 & 0.03 & -0.0 \\
 &  & RMSE & (1.19) & (0.96) & (0.3) & (0.21) & (0.12) \\
 & U & Bias & 0.85 & 0.29 & 0.09 & 0.06 & 0.01 \\
 &  & RMSE & (2.0) & (0.85) & (0.46) & (0.29) & (0.19) \\
 & Non & Bias & 0.51 & 0.25 & 0.04 & 0.02 & -0.0 \\
 &  & RMSE & (1.19) & (0.96) & (0.28) & (0.21) & (0.12) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.61 & 15.01 & 21.99 & 35.74 & 71.11 \\
 & U,T & Bias & 0.08 & 1.18 & 1.47 & 0.96 & 0.37 \\
 &  & RMSE & (3.49) & (3.28) & (3.45) & (2.41) & (1.1) \\
 & T & Bias & 0.32 & 0.14 & 0.07 & 0.04 & 0.01 \\
 &  & RMSE & (1.03) & (0.71) & (0.36) & (0.18) & (0.09) \\
 & U & Bias & 0.21 & 1.08 & 1.55 & 1.02 & 0.37 \\
 &  & RMSE & (3.66) & (3.18) & (3.54) & (2.44) & (1.11) \\
 & Non & Bias & 0.32 & 0.13 & 0.03 & 0.04 & 0.01 \\
 &  & RMSE & (1.03) & (0.69) & (0.22) & (0.16) & (0.09) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 9.73 & 19.44 & 28.91 & 47.78 & 95.25 \\
 & U,T & Bias & -1.2 & -0.67 & 0.32 & 1.09 & 1.34 \\
 &  & RMSE & (5.1) & (5.66) & (5.27) & (4.98) & (3.67) \\
 & T & Bias & -2.52 & -2.09 & -1.0 & -0.02 & 0.02 \\
 &  & RMSE & (4.45) & (4.16) & (3.1) & (1.3) & (0.28) \\
 & U & Bias & -1.2 & -0.67 & 0.04 & 1.06 & 1.52 \\
 &  & RMSE & (5.1) & (5.66) & (5.23) & (5.0) & (3.99) \\
 & Non & Bias & -2.52 & -2.09 & -0.99 & -0.0 & 0.02 \\
 &  & RMSE & (4.45) & (4.16) & (3.1) & (1.3) & (0.26) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta1_without_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.09 & 0.58 & 0.26 & 0.25 & 0.18 \\
 &  & RMSE & (0.41) & (1.11) & (0.65) & (0.44) & (0.36) \\
 & T & Bias & 0.29 & 0.61 & 0.29 & 0.25 & 0.18 \\
 &  & RMSE & (1.12) & (1.14) & (0.71) & (0.46) & (0.35) \\
 & U & Bias & 0.29 & 0.64 & 0.29 & 0.25 & 0.18 \\
 &  & RMSE & (1.12) & (1.15) & (0.71) & (0.47) & (0.36) \\
 & Non & Bias & 0.29 & 0.64 & 0.29 & 0.25 & 0.18 \\
 &  & RMSE & (1.12) & (1.15) & (0.71) & (0.47) & (0.36) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.03 \\
 & U,T & Bias & 1.37 & 0.68 & 0.71 & 0.68 & 0.52 \\
 &  & RMSE & (2.69) & (1.17) & (1.03) & (0.9) & (0.73) \\
 & T & Bias & 1.45 & 0.7 & 0.71 & 0.69 & 0.54 \\
 &  & RMSE & (2.72) & (1.18) & (1.02) & (0.92) & (0.75) \\
 & U & Bias & 1.46 & 0.74 & 0.74 & 0.69 & 0.54 \\
 &  & RMSE & (2.73) & (1.22) & (1.03) & (0.92) & (0.75) \\
 & Non & Bias & 1.43 & 0.74 & 0.74 & 0.69 & 0.54 \\
 &  & RMSE & (2.71) & (1.22) & (1.03) & (0.92) & (0.75) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.91 & 3.17 & 4.59 & 6.85 & 12.71 \\
 & U,T & Bias & 1.43 & 1.17 & 0.86 & 0.68 & 0.8 \\
 &  & RMSE & (2.51) & (1.74) & (1.15) & (0.83) & (0.96) \\
 & T & Bias & 1.44 & 0.95 & 0.78 & 0.74 & 0.7 \\
 &  & RMSE & (2.38) & (1.36) & (1.07) & (0.98) & (0.87) \\
 & U & Bias & 1.46 & 1.05 & 0.86 & 0.69 & 0.78 \\
 &  & RMSE & (2.39) & (1.61) & (1.13) & (0.87) & (0.96) \\
 & Non & Bias & 1.43 & 0.96 & 0.77 & 0.75 & 0.73 \\
 &  & RMSE & (2.38) & (1.36) & (1.07) & (0.98) & (0.9) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.57 & 11.12 & 15.81 & 25.85 & 50.68 \\
 & U,T & Bias & 1.83 & 1.51 & 0.73 & 0.6 & 0.63 \\
 &  & RMSE & (3.31) & (2.54) & (1.2) & (0.89) & (0.82) \\
 & T & Bias & 1.15 & 0.84 & 0.62 & 0.69 & 0.5 \\
 &  & RMSE & (2.35) & (1.18) & (0.83) & (0.91) & (0.69) \\
 & U & Bias & 1.81 & 1.5 & 0.75 & 0.61 & 0.61 \\
 &  & RMSE & (3.2) & (2.53) & (1.35) & (0.9) & (0.79) \\
 & Non & Bias & 1.14 & 0.82 & 0.64 & 0.69 & 0.46 \\
 &  & RMSE & (2.34) & (1.16) & (0.85) & (0.91) & (0.61) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.87 & 14.94 & 22.2 & 36.22 & 72.12 \\
 & U,T & Bias & 2.02 & 2.15 & 1.24 & 0.65 & 0.55 \\
 &  & RMSE & (4.1) & (3.48) & (2.17) & (1.08) & (0.78) \\
 & T & Bias & 0.41 & 0.57 & 0.47 & 0.46 & 0.52 \\
 &  & RMSE & (2.21) & (0.89) & (0.67) & (0.63) & (0.69) \\
 & U & Bias & 2.04 & 2.24 & 1.28 & 0.67 & 0.55 \\
 &  & RMSE & (4.1) & (3.56) & (2.23) & (1.1) & (0.77) \\
 & Non & Bias & 0.41 & 0.57 & 0.5 & 0.46 & 0.5 \\
 &  & RMSE & (2.21) & (0.89) & (0.71) & (0.63) & (0.62) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta1_without_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 1.13 & 0.55 & 0.29 & 0.23 & 0.13 \\
 &  & RMSE & (2.28) & (1.22) & (0.69) & (0.46) & (0.27) \\
 & T & Bias & 1.22 & 0.55 & 0.29 & 0.24 & 0.13 \\
 &  & RMSE & (2.42) & (1.22) & (0.69) & (0.46) & (0.28) \\
 & U & Bias & 1.31 & 0.56 & 0.29 & 0.23 & 0.13 \\
 &  & RMSE & (2.51) & (1.22) & (0.69) & (0.46) & (0.28) \\
 & Non & Bias & 1.18 & 0.56 & 0.29 & 0.23 & 0.13 \\
 &  & RMSE & (2.34) & (1.22) & (0.69) & (0.46) & (0.28) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 1.08 & 0.69 & 0.47 & 0.35 & 0.38 \\
 &  & RMSE & (2.68) & (1.3) & (0.87) & (0.6) & (0.55) \\
 & T & Bias & 1.15 & 0.69 & 0.47 & 0.35 & 0.39 \\
 &  & RMSE & (2.74) & (1.3) & (0.87) & (0.6) & (0.55) \\
 & U & Bias & 1.16 & 0.69 & 0.47 & 0.36 & 0.38 \\
 &  & RMSE & (2.74) & (1.3) & (0.87) & (0.61) & (0.55) \\
 & Non & Bias & 1.16 & 0.68 & 0.47 & 0.36 & 0.38 \\
 &  & RMSE & (2.74) & (1.3) & (0.87) & (0.61) & (0.55) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.72 & 3.32 & 4.51 & 6.9 & 13.04 \\
 & U,T & Bias & 0.67 & 0.49 & 0.16 & 0.24 & 0.14 \\
 &  & RMSE & (1.49) & (1.33) & (0.41) & (0.41) & (0.3) \\
 & T & Bias & 0.73 & 0.35 & 0.2 & 0.2 & 0.15 \\
 &  & RMSE & (1.63) & (0.67) & (0.44) & (0.37) & (0.31) \\
 & U & Bias & 0.71 & 0.48 & 0.2 & 0.23 & 0.14 \\
 &  & RMSE & (1.52) & (1.31) & (0.52) & (0.4) & (0.3) \\
 & Non & Bias & 0.78 & 0.35 & 0.19 & 0.19 & 0.15 \\
 &  & RMSE & (1.74) & (0.67) & (0.44) & (0.37) & (0.3) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.9 & 11.2 & 16.12 & 26.05 & 50.61 \\
 & U,T & Bias & 0.88 & 0.81 & 0.44 & 0.23 & 0.1 \\
 &  & RMSE & (3.01) & (1.97) & (1.42) & (0.58) & (0.24) \\
 & T & Bias & 0.31 & 0.15 & 0.1 & 0.12 & 0.1 \\
 &  & RMSE & (1.43) & (0.41) & (0.29) & (0.28) & (0.24) \\
 & U & Bias & 0.83 & 0.84 & 0.45 & 0.27 & 0.09 \\
 &  & RMSE & (3.01) & (1.98) & (1.42) & (0.67) & (0.24) \\
 & Non & Bias & 0.3 & 0.12 & 0.09 & 0.12 & 0.08 \\
 &  & RMSE & (1.43) & (0.38) & (0.28) & (0.27) & (0.22) \\
 &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.58 & 14.9 & 22.12 & 36.68 & 72.29 \\
 & U,T & Bias & 0.4 & 0.67 & 0.43 & 0.27 & 0.21 \\
 &  & RMSE & (4.27) & (3.01) & (1.58) & (0.78) & (0.47) \\
 & T & Bias & -0.07 & 0.19 & 0.11 & 0.08 & 0.09 \\
 &  & RMSE & (2.07) & (0.51) & (0.35) & (0.29) & (0.2) \\
 & U & Bias & 0.51 & 0.66 & 0.43 & 0.31 & 0.21 \\
 &  & RMSE & (4.31) & (3.01) & (1.58) & (0.79) & (0.48) \\
 & Non & Bias & -0.08 & 0.17 & 0.09 & 0.06 & 0.08 \\
 &  & RMSE & (2.07) & (0.51) & (0.32) & (0.27) & (0.2) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta2_with_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_2$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 4.44 & 4.18 & 4.32 & 4.34 & 4.41 \\
 &  & RMSE & (5.37) & (5.04) & (5.12) & (5.11) & (5.29) \\
 & T & Bias & 4.36 & 4.22 & 4.29 & 4.28 & 4.41 \\
 &  & RMSE & (5.31) & (5.08) & (5.08) & (5.04) & (5.29) \\
 & U & Bias & 4.37 & 4.13 & 4.33 & 4.28 & 4.55 \\
 &  & RMSE & (5.3) & (5.0) & (5.12) & (5.04) & (5.41) \\
 & Non & Bias & 4.42 & 4.17 & 4.33 & 4.28 & 4.55 \\
 &  & RMSE & (5.32) & (5.04) & (5.12) & (5.04) & (5.41) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 5.23 & 5.17 & 5.3 & 5.26 & 5.59 \\
 &  & RMSE & (5.93) & (5.9) & (5.97) & (5.88) & (6.31) \\
 & T & Bias & 5.26 & 5.18 & 5.3 & 5.26 & 5.59 \\
 &  & RMSE & (5.97) & (5.9) & (5.97) & (5.88) & (6.31) \\
 & U & Bias & 5.32 & 5.09 & 5.36 & 5.27 & 5.62 \\
 &  & RMSE & (6.02) & (5.82) & (6.02) & (5.89) & (6.34) \\
 & Non & Bias & 5.3 & 5.11 & 5.34 & 5.27 & 5.62 \\
 &  & RMSE & (6.0) & (5.85) & (6.01) & (5.89) & (6.34) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 2.44 & 4.77 & 6.51 & 10.48 & 19.2 \\
 & U,T & Bias & 2.62 & 3.79 & 4.39 & 3.41 & 3.78 \\
 &  & RMSE & (4.83) & (5.61) & (5.87) & (4.85) & (5.3) \\
 & T & Bias & 1.4 & 1.93 & 1.54 & 1.3 & 1.16 \\
 &  & RMSE & (3.62) & (4.13) & (3.03) & (2.64) & (2.53) \\
 & U & Bias & 2.3 & 3.77 & 4.16 & 3.31 & 3.52 \\
 &  & RMSE & (4.47) & (5.6) & (5.7) & (4.77) & (5.01) \\
 & Non & Bias & 1.4 & 1.88 & 1.53 & 1.13 & 1.07 \\
 &  & RMSE & (3.62) & (4.06) & (3.01) & (2.36) & (2.4) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.56 & 14.89 & 21.98 & 35.88 & 71.27 \\
 & U,T & Bias & 2.76 & 5.04 & 5.36 & 5.74 & 6.41 \\
 &  & RMSE & (5.47) & (6.74) & (6.8) & (6.84) & (7.25) \\
 & T & Bias & -0.95 & -0.45 & -0.06 & -0.09 & -0.12 \\
 &  & RMSE & (2.12) & (1.37) & (0.58) & (0.55) & (0.62) \\
 & U & Bias & 2.43 & 4.97 & 5.43 & 5.68 & 6.4 \\
 &  & RMSE & (5.24) & (6.72) & (6.9) & (6.81) & (7.27) \\
 & Non & Bias & -0.94 & -0.44 & -0.07 & -0.08 & -0.1 \\
 &  & RMSE & (2.11) & (1.36) & (0.58) & (0.55) & (0.62) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 9.77 & 19.47 & 28.86 & 47.81 & 95.1 \\
 & U,T & Bias & 0.88 & 3.5 & 3.7 & 4.61 & 5.48 \\
 &  & RMSE & (5.67) & (6.5) & (6.34) & (6.76) & (7.25) \\
 & T & Bias & -2.25 & -1.71 & -1.66 & -0.6 & -0.18 \\
 &  & RMSE & (3.5) & (3.0) & (2.77) & (1.61) & (0.92) \\
 & U & Bias & 0.81 & 3.35 & 3.73 & 4.57 & 5.55 \\
 &  & RMSE & (5.65) & (6.38) & (6.37) & (6.7) & (7.32) \\
 & Non & Bias & -2.25 & -1.71 & -1.62 & -0.59 & -0.19 \\
 &  & RMSE & (3.5) & (3.0) & (2.72) & (1.61) & (0.9) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta2_with_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_2$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & -0.12 & -0.86 & -0.75 & -1.72 & -1.77 \\
 &  & RMSE & (5.48) & (5.32) & (5.77) & (5.85) & (5.98) \\
 & T & Bias & -0.12 & -0.83 & -0.75 & -1.72 & -1.77 \\
 &  & RMSE & (5.48) & (5.29) & (5.77) & (5.85) & (5.98) \\
 & U & Bias & -0.08 & -0.92 & -0.74 & -1.7 & -1.58 \\
 &  & RMSE & (5.35) & (5.26) & (5.75) & (5.86) & (5.98) \\
 & Non & Bias & -0.04 & -0.92 & -0.74 & -1.7 & -1.58 \\
 &  & RMSE & (5.5) & (5.26) & (5.75) & (5.86) & (5.98) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.7 & -0.12 & 0.25 & -0.82 & -0.93 \\
 &  & RMSE & (5.45) & (5.02) & (5.73) & (5.69) & (5.83) \\
 & T & Bias & 0.59 & -0.12 & 0.25 & -0.77 & -0.93 \\
 &  & RMSE & (5.5) & (5.02) & (5.73) & (5.68) & (5.83) \\
 & U & Bias & 0.68 & -0.17 & 0.26 & -0.7 & -0.54 \\
 &  & RMSE & (5.42) & (4.94) & (5.71) & (5.65) & (5.84) \\
 & Non & Bias & 0.68 & -0.17 & 0.26 & -0.7 & -0.54 \\
 &  & RMSE & (5.42) & (4.94) & (5.71) & (5.65) & (5.84) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 2.59 & 4.68 & 6.33 & 10.27 & 18.64 \\
 & U,T & Bias & -1.87 & -2.63 & -1.95 & -1.62 & -1.47 \\
 &  & RMSE & (3.97) & (5.64) & (5.52) & (5.52) & (5.34) \\
 & T & Bias & -2.58 & -4.96 & -4.69 & -4.59 & -4.48 \\
 &  & RMSE & (3.57) & (5.57) & (5.33) & (5.32) & (5.17) \\
 & U & Bias & -1.74 & -2.62 & -2.49 & -1.91 & -1.93 \\
 &  & RMSE & (4.08) & (5.6) & (5.52) & (5.32) & (5.22) \\
 & Non & Bias & -2.61 & -5.06 & -4.84 & -4.73 & -4.69 \\
 &  & RMSE & (3.59) & (5.63) & (5.42) & (5.39) & (5.31) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.61 & 15.01 & 21.99 & 35.74 & 71.11 \\
 & U,T & Bias & 0.85 & 1.45 & 1.22 & 2.18 & 2.34 \\
 &  & RMSE & (5.14) & (6.27) & (5.5) & (5.79) & (6.14) \\
 & T & Bias & -2.4 & -4.49 & -4.12 & -4.23 & -4.44 \\
 &  & RMSE & (3.42) & (5.01) & (4.69) & (4.82) & (5.01) \\
 & U & Bias & 0.54 & 1.29 & 1.18 & 2.0 & 2.68 \\
 &  & RMSE & (4.97) & (6.1) & (5.64) & (5.72) & (6.3) \\
 & Non & Bias & -2.4 & -4.61 & -4.28 & -4.45 & -4.54 \\
 &  & RMSE & (3.42) & (5.06) & (4.8) & (4.95) & (5.03) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 9.73 & 19.44 & 28.91 & 47.78 & 95.25 \\
 & U,T & Bias & 0.34 & 2.78 & 2.45 & 1.79 & 2.89 \\
 &  & RMSE & (5.65) & (6.5) & (6.12) & (6.06) & (6.14) \\
 & T & Bias & -2.49 & -3.52 & -3.65 & -3.39 & -3.72 \\
 &  & RMSE & (4.14) & (4.34) & (4.23) & (4.01) & (4.31) \\
 & U & Bias & 0.34 & 2.78 & 2.35 & 1.61 & 2.79 \\
 &  & RMSE & (5.65) & (6.5) & (6.1) & (5.95) & (6.16) \\
 & Non & Bias & -2.49 & -3.52 & -3.79 & -3.57 & -3.92 \\
 &  & RMSE & (4.14) & (4.34) & (4.34) & (4.1) & (4.42) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta2_without_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_2$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.18 & 1.07 & 0.63 & 0.46 & 0.33 \\
 &  & RMSE & (0.48) & (1.99) & (1.23) & (0.84) & (0.65) \\
 & T & Bias & 0.25 & 1.2 & 0.73 & 0.51 & 0.34 \\
 &  & RMSE & (0.66) & (2.18) & (1.37) & (0.9) & (0.65) \\
 & U & Bias & 0.25 & 1.26 & 0.74 & 0.51 & 0.36 \\
 &  & RMSE & (0.66) & (2.22) & (1.37) & (0.9) & (0.68) \\
 & Non & Bias & 0.25 & 1.26 & 0.74 & 0.51 & 0.36 \\
 &  & RMSE & (0.66) & (2.22) & (1.37) & (0.9) & (0.68) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.03 \\
 & U,T & Bias & 0.38 & 0.17 & 0.05 & 0.07 & 0.07 \\
 &  & RMSE & (1.35) & (0.55) & (0.31) & (0.21) & (0.18) \\
 & T & Bias & 0.36 & 0.18 & 0.04 & 0.07 & 0.07 \\
 &  & RMSE & (1.36) & (0.56) & (0.29) & (0.2) & (0.19) \\
 & U & Bias & 0.37 & 0.16 & 0.03 & 0.07 & 0.07 \\
 &  & RMSE & (1.36) & (0.55) & (0.29) & (0.2) & (0.19) \\
 & Non & Bias & 0.37 & 0.16 & 0.03 & 0.07 & 0.07 \\
 &  & RMSE & (1.35) & (0.55) & (0.29) & (0.2) & (0.19) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 1.91 & 3.17 & 4.59 & 6.85 & 12.71 \\
 & U,T & Bias & -0.41 & -0.14 & 0.06 & 0.13 & 0.15 \\
 &  & RMSE & (1.28) & (0.62) & (0.4) & (0.28) & (0.31) \\
 & T & Bias & -0.55 & -0.14 & 0.03 & 0.09 & 0.13 \\
 &  & RMSE & (1.23) & (0.63) & (0.4) & (0.31) & (0.31) \\
 & U & Bias & -0.49 & -0.09 & 0.03 & 0.13 & 0.16 \\
 &  & RMSE & (1.34) & (0.58) & (0.38) & (0.3) & (0.34) \\
 & Non & Bias & -0.54 & -0.15 & 0.03 & 0.08 & 0.13 \\
 &  & RMSE & (1.23) & (0.63) & (0.39) & (0.31) & (0.32) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 5.57 & 11.12 & 15.81 & 25.85 & 50.68 \\
 & U,T & Bias & -0.61 & -0.35 & 0.12 & 0.22 & 0.34 \\
 &  & RMSE & (3.02) & (1.17) & (0.69) & (0.61) & (0.56) \\
 & T & Bias & -1.27 & -0.45 & -0.14 & -0.14 & 0.02 \\
 &  & RMSE & (2.5) & (1.05) & (0.61) & (0.57) & (0.58) \\
 & U & Bias & -0.77 & -0.34 & 0.14 & 0.2 & 0.37 \\
 &  & RMSE & (2.87) & (1.12) & (0.78) & (0.63) & (0.55) \\
 & Non & Bias & -1.25 & -0.43 & -0.14 & -0.14 & 0.08 \\
 &  & RMSE & (2.51) & (1.03) & (0.61) & (0.57) & (0.45) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 7.87 & 14.94 & 22.2 & 36.22 & 72.12 \\
 & U,T & Bias & -0.02 & -0.26 & -0.2 & 0.42 & 0.31 \\
 &  & RMSE & (3.87) & (3.41) & (2.28) & (0.97) & (0.81) \\
 & T & Bias & -1.47 & -0.57 & -0.26 & -0.07 & -0.15 \\
 &  & RMSE & (2.67) & (1.49) & (0.94) & (0.77) & (0.8) \\
 & U & Bias & 0.03 & -0.35 & -0.19 & 0.36 & 0.32 \\
 &  & RMSE & (3.79) & (3.42) & (2.29) & (0.9) & (0.81) \\
 & Non & Bias & -1.47 & -0.57 & -0.3 & -0.05 & -0.11 \\
 &  & RMSE & (2.67) & (1.49) & (0.98) & (0.76) & (0.65) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta2_without_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_2$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 1.73 & 1.0 & 0.7 & 0.49 & 0.3 \\
 &  & RMSE & (3.18) & (2.01) & (1.4) & (0.86) & (0.63) \\
 & T & Bias & 1.76 & 1.0 & 0.7 & 0.49 & 0.32 \\
 &  & RMSE & (3.21) & (2.01) & (1.4) & (0.86) & (0.65) \\
 & U & Bias & 1.74 & 1.01 & 0.7 & 0.49 & 0.33 \\
 &  & RMSE & (3.21) & (2.01) & (1.4) & (0.86) & (0.65) \\
 & Non & Bias & 1.72 & 1.01 & 0.7 & 0.49 & 0.33 \\
 &  & RMSE & (3.18) & (2.01) & (1.4) & (0.86) & (0.65) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.13 & 0.14 & -0.01 & 0.01 & -0.01 \\
 &  & RMSE & (1.91) & (0.59) & (0.31) & (0.21) & (0.17) \\
 & T & Bias & 0.11 & 0.14 & -0.01 & 0.0 & -0.0 \\
 &  & RMSE & (1.94) & (0.59) & (0.31) & (0.21) & (0.17) \\
 & U & Bias & 0.12 & 0.13 & -0.01 & 0.01 & -0.01 \\
 &  & RMSE & (1.95) & (0.59) & (0.31) & (0.21) & (0.17) \\
 & Non & Bias & 0.11 & 0.13 & -0.01 & 0.01 & -0.01 \\
 &  & RMSE & (1.95) & (0.59) & (0.31) & (0.21) & (0.17) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 1.72 & 3.32 & 4.51 & 6.9 & 13.04 \\
 & U,T & Bias & -1.38 & -0.66 & -0.26 & -0.33 & -0.22 \\
 &  & RMSE & (2.48) & (1.24) & (0.59) & (0.6) & (0.37) \\
 & T & Bias & -1.24 & -0.54 & -0.27 & -0.32 & -0.27 \\
 &  & RMSE & (2.14) & (0.84) & (0.5) & (0.56) & (0.45) \\
 & U & Bias & -1.43 & -0.69 & -0.3 & -0.3 & -0.26 \\
 &  & RMSE & (2.51) & (1.25) & (0.71) & (0.58) & (0.42) \\
 & Non & Bias & -1.3 & -0.53 & -0.25 & -0.31 & -0.27 \\
 &  & RMSE & (2.27) & (0.84) & (0.5) & (0.56) & (0.45) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 5.9 & 11.2 & 16.12 & 26.05 & 50.61 \\
 & U,T & Bias & -1.47 & -1.68 & -1.04 & -0.64 & -0.2 \\
 &  & RMSE & (3.0) & (2.94) & (2.09) & (1.48) & (0.59) \\
 & T & Bias & -1.29 & -0.62 & -0.48 & -0.36 & -0.26 \\
 &  & RMSE & (2.22) & (0.99) & (0.76) & (0.63) & (0.5) \\
 & U & Bias & -1.32 & -1.73 & -1.01 & -0.69 & -0.22 \\
 &  & RMSE & (3.17) & (2.94) & (2.04) & (1.56) & (0.63) \\
 & Non & Bias & -1.3 & -0.58 & -0.48 & -0.36 & -0.24 \\
 &  & RMSE & (2.23) & (0.98) & (0.75) & (0.64) & (0.47) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 7.58 & 14.9 & 22.12 & 36.68 & 72.29 \\
 & U,T & Bias & -0.63 & -1.07 & -1.5 & -0.68 & -0.79 \\
 &  & RMSE & (4.21) & (3.08) & (2.98) & (1.91) & (1.68) \\
 & T & Bias & -1.79 & -0.94 & -0.62 & -0.43 & -0.37 \\
 &  & RMSE & (2.77) & (1.72) & (1.26) & (0.82) & (0.64) \\
 & U & Bias & -0.77 & -1.08 & -1.5 & -0.76 & -0.8 \\
 &  & RMSE & (4.16) & (3.08) & (2.98) & (1.94) & (1.69) \\
 & Non & Bias & -1.82 & -0.93 & -0.59 & -0.42 & -0.39 \\
 &  & RMSE & (2.77) & (1.71) & (1.22) & (0.82) & (0.63) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta_without_dummy_with_IR_penalty_1.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc|lccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  & $\beta_2$ &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 0.16 & 0.45 & 0.27 & 0.22 & 0.11 &  & 0.22 & 0.84 & 0.69 & 0.49 & 0.32 \\
 &  & RMSE & (0.65) & (1.23) & (0.66) & (0.45) & (0.25) &  & (0.46) & (1.96) & (1.3) & (0.86) & (0.64) \\
 & T & Bias & 0.1 & 0.45 & 0.28 & 0.22 & 0.12 &  & 0.23 & 0.84 & 0.68 & 0.49 & 0.33 \\
 &  & RMSE & (0.4) & (1.22) & (0.67) & (0.46) & (0.27) &  & (0.41) & (1.96) & (1.3) & (0.86) & (0.65) \\
 & U & Bias & 0.26 & 0.46 & 0.28 & 0.22 & 0.12 &  & 0.26 & 0.85 & 0.68 & 0.49 & 0.33 \\
 &  & RMSE & (1.08) & (1.23) & (0.67) & (0.46) & (0.27) &  & (0.53) & (1.96) & (1.3) & (0.86) & (0.65) \\
 & Non & Bias & 0.21 & 0.45 & 0.28 & 0.22 & 0.12 &  & 0.27 & 0.85 & 0.68 & 0.49 & 0.33 \\
 &  & RMSE & (0.96) & (1.23) & (0.67) & (0.46) & (0.27) &  & (0.52) & (1.96) & (1.3) & (0.86) & (0.65) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 & 0.0 & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.33 & 0.45 & 0.46 & 0.35 & 0.39 &  & 0.06 & 0.07 & 0.01 & 0.01 & -0.02 \\
 &  & RMSE & (0.86) & (0.97) & (0.84) & (0.58) & (0.58) &  & (0.96) & (0.47) & (0.26) & (0.21) & (0.16) \\
 & T & Bias & 0.29 & 0.45 & 0.46 & 0.34 & 0.39 &  & 0.09 & 0.07 & 0.01 & 0.02 & -0.01 \\
 &  & RMSE & (0.72) & (0.97) & (0.84) & (0.58) & (0.58) &  & (0.89) & (0.47) & (0.26) & (0.2) & (0.17) \\
 & U & Bias & 0.29 & 0.45 & 0.47 & 0.35 & 0.39 &  & 0.1 & 0.08 & 0.01 & 0.02 & -0.0 \\
 &  & RMSE & (0.72) & (0.97) & (0.84) & (0.58) & (0.58) &  & (0.9) & (0.47) & (0.26) & (0.2) & (0.16) \\
 & Non & Bias & 0.37 & 0.45 & 0.47 & 0.35 & 0.39 &  & 0.09 & 0.07 & 0.01 & 0.02 & -0.0 \\
 &  & RMSE & (0.97) & (0.97) & (0.84) & (0.58) & (0.58) &  & (0.97) & (0.47) & (0.26) & (0.2) & (0.16) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.74 & 3.21 & 4.34 & 6.92 & 12.43 & -1.0 & 1.74 & 3.21 & 4.34 & 6.92 & 12.43 \\
 & U,T & Bias & 1.17 & 0.32 & 0.24 & 0.22 & 0.14 &  & -0.87 & -0.26 & -0.18 & -0.24 & -0.13 \\
 &  & RMSE & (2.33) & (0.59) & (0.46) & (0.43) & (0.29) &  & (1.91) & (0.51) & (0.41) & (0.47) & (0.35) \\
 & T & Bias & 1.35 & 0.37 & 0.25 & 0.23 & 0.15 &  & -0.93 & -0.22 & -0.16 & -0.18 & -0.14 \\
 &  & RMSE & (2.51) & (0.95) & (0.56) & (0.41) & (0.28) &  & (1.98) & (0.48) & (0.54) & (0.46) & (0.33) \\
 & U & Bias & 1.24 & 0.32 & 0.23 & 0.22 & 0.15 &  & -0.91 & -0.25 & -0.16 & -0.21 & -0.13 \\
 &  & RMSE & (2.41) & (0.59) & (0.45) & (0.43) & (0.3) &  & (1.94) & (0.51) & (0.4) & (0.45) & (0.35) \\
 & Non & Bias & 1.36 & 0.38 & 0.25 & 0.22 & 0.15 &  & -0.94 & -0.22 & -0.15 & -0.19 & -0.13 \\
 &  & RMSE & (2.52) & (0.96) & (0.56) & (0.42) & (0.28) &  & (1.99) & (0.48) & (0.54) & (0.46) & (0.34) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.4 & 10.61 & 15.91 & 25.62 & 50.34 & -2.0 & 5.4 & 10.61 & 15.91 & 25.62 & 50.34 \\
 & U,T & Bias & 0.44 & 0.12 & 0.16 & 0.17 & 0.11 &  & -0.81 & -0.28 & -0.3 & -0.33 & -0.2 \\
 &  & RMSE & (1.6) & (0.37) & (0.36) & (0.31) & (0.24) &  & (1.77) & (0.63) & (0.65) & (0.6) & (0.48) \\
 & T & Bias & 1.01 & 0.43 & 0.59 & 0.32 & 0.18 &  & -0.65 & -0.36 & -0.22 & -0.05 & -0.03 \\
 &  & RMSE & (2.32) & (0.94) & (1.5) & (0.75) & (0.36) &  & (2.49) & (1.0) & (0.98) & (0.83) & (0.46) \\
 & U & Bias & 0.42 & 0.11 & 0.16 & 0.18 & 0.11 &  & -0.78 & -0.26 & -0.29 & -0.32 & -0.19 \\
 &  & RMSE & (1.6) & (0.34) & (0.36) & (0.31) & (0.23) &  & (1.77) & (0.59) & (0.64) & (0.6) & (0.45) \\
 & Non & Bias & 0.93 & 0.45 & 0.59 & 0.32 & 0.17 &  & -0.7 & -0.35 & -0.23 & -0.05 & -0.02 \\
 &  & RMSE & (2.27) & (0.97) & (1.51) & (0.75) & (0.36) &  & (2.33) & (1.01) & (0.99) & (0.83) & (0.45) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.57 & 14.94 & 22.19 & 36.09 & 71.83 & -3.0 & 7.57 & 14.94 & 22.19 & 36.09 & 71.83 \\
 & U,T & Bias & 0.07 & 0.25 & 0.14 & 0.13 & 0.09 &  & -1.16 & -0.52 & -0.4 & -0.31 & -0.25 \\
 &  & RMSE & (2.02) & (0.54) & (0.39) & (0.27) & (0.2) &  & (2.34) & (1.19) & (0.97) & (0.65) & (0.55) \\
 & T & Bias & 1.08 & 1.32 & 0.56 & 0.18 & 0.26 &  & 0.16 & 0.04 & -0.23 & -0.02 & -0.02 \\
 &  & RMSE & (3.04) & (2.58) & (1.14) & (0.4) & (0.54) &  & (3.67) & (2.89) & (1.61) & (0.53) & (0.86) \\
 & U & Bias & 0.08 & 0.22 & 0.14 & 0.11 & 0.08 &  & -1.18 & -0.48 & -0.41 & -0.29 & -0.25 \\
 &  & RMSE & (2.02) & (0.53) & (0.36) & (0.25) & (0.2) &  & (2.33) & (1.17) & (0.92) & (0.63) & (0.53) \\
 & Non & Bias & 1.13 & 1.36 & 0.58 & 0.17 & 0.26 &  & 0.16 & 0.01 & -0.24 & -0.02 & -0.01 \\
 &  & RMSE & (3.03) & (2.6) & (1.18) & (0.4) & (0.55) &  & (3.66) & (2.9) & (1.62) & (0.54) & (0.86) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_two_param_beta_without_dummy_without_IR_penalty_1.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc|lccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 &  & 10 & 20 & 30 & 50 & 100 \\
$\beta_1$ &  &  &  &  &  &  &  & $\beta_2$ &  &  &  &  &  \\
\midrule 
0.5 & unmatched & Mean Num & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
 & U,T & Bias & 1.4 & 0.42 & 0.25 & 0.23 & 0.12 &  & 1.9 & 0.81 & 0.66 & 0.49 & 0.31 \\
 &  & RMSE & (2.65) & (1.16) & (0.6) & (0.46) & (0.26) &  & (3.33) & (1.88) & (1.36) & (0.86) & (0.63) \\
 & T & Bias & 1.44 & 0.42 & 0.25 & 0.23 & 0.13 &  & 1.88 & 0.81 & 0.66 & 0.49 & 0.33 \\
 &  & RMSE & (2.67) & (1.16) & (0.6) & (0.46) & (0.28) &  & (3.33) & (1.88) & (1.36) & (0.86) & (0.65) \\
 & U & Bias & 1.49 & 0.43 & 0.24 & 0.23 & 0.13 &  & 1.88 & 0.82 & 0.66 & 0.49 & 0.33 \\
 &  & RMSE & (2.73) & (1.16) & (0.6) & (0.46) & (0.28) &  & (3.33) & (1.88) & (1.36) & (0.86) & (0.65) \\
 & Non & Bias & 1.49 & 0.43 & 0.25 & 0.23 & 0.13 &  & 1.88 & 0.82 & 0.65 & 0.49 & 0.33 \\
 &  & RMSE & (2.73) & (1.16) & (0.6) & (0.46) & (0.28) &  & (3.33) & (1.88) & (1.36) & (0.86) & (0.65) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 & 0.0 & 0.01 & 0.0 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.55 & 0.46 & 0.46 & 0.35 & 0.39 &  & -0.18 & 0.05 & -0.01 & 0.01 & -0.01 \\
 &  & RMSE & (1.53) & (1.0) & (0.87) & (0.6) & (0.55) &  & (1.6) & (0.48) & (0.31) & (0.21) & (0.17) \\
 & T & Bias & 0.55 & 0.45 & 0.46 & 0.35 & 0.39 &  & -0.18 & 0.04 & -0.01 & 0.01 & -0.01 \\
 &  & RMSE & (1.53) & (1.0) & (0.87) & (0.6) & (0.55) &  & (1.6) & (0.48) & (0.31) & (0.21) & (0.17) \\
 & U & Bias & 0.55 & 0.46 & 0.46 & 0.36 & 0.39 &  & -0.17 & 0.03 & -0.01 & 0.01 & -0.01 \\
 &  & RMSE & (1.53) & (1.0) & (0.87) & (0.61) & (0.55) &  & (1.61) & (0.48) & (0.31) & (0.21) & (0.17) \\
 & Non & Bias & 0.55 & 0.45 & 0.46 & 0.36 & 0.39 &  & -0.17 & 0.03 & -0.01 & 0.01 & -0.01 \\
 &  & RMSE & (1.53) & (1.0) & (0.87) & (0.61) & (0.55) &  & (1.61) & (0.48) & (0.31) & (0.21) & (0.17) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 1.7 & 3.11 & 4.69 & 6.64 & 13.01 & -1.0 & 1.7 & 3.11 & 4.69 & 6.64 & 13.01 \\
 & U,T & Bias & 0.57 & 0.35 & 0.2 & 0.21 & 0.15 &  & -0.89 & -0.54 & -0.27 & -0.33 & -0.27 \\
 &  & RMSE & (1.48) & (0.67) & (0.44) & (0.38) & (0.31) &  & (1.73) & (0.84) & (0.5) & (0.58) & (0.44) \\
 & T & Bias & 0.61 & 0.45 & 0.17 & 0.23 & 0.15 &  & -1.1 & -0.49 & -0.28 & -0.29 & -0.23 \\
 &  & RMSE & (1.46) & (1.3) & (0.42) & (0.4) & (0.3) &  & (2.21) & (0.85) & (0.61) & (0.57) & (0.4) \\
 & U & Bias & 0.62 & 0.35 & 0.19 & 0.19 & 0.15 &  & -0.95 & -0.53 & -0.25 & -0.31 & -0.27 \\
 &  & RMSE & (1.6) & (0.67) & (0.44) & (0.37) & (0.3) &  & (1.89) & (0.84) & (0.5) & (0.56) & (0.45) \\
 & Non & Bias & 0.6 & 0.46 & 0.21 & 0.23 & 0.15 &  & -1.12 & -0.5 & -0.3 & -0.31 & -0.26 \\
 &  & RMSE & (1.43) & (1.3) & (0.52) & (0.39) & (0.3) &  & (2.24) & (0.86) & (0.71) & (0.59) & (0.43) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 5.56 & 10.89 & 15.94 & 25.3 & 49.92 & -2.0 & 5.56 & 10.89 & 15.94 & 25.3 & 49.92 \\
 & U,T & Bias & 0.34 & 0.15 & 0.1 & 0.12 & 0.1 &  & -1.38 & -0.62 & -0.48 & -0.36 & -0.26 \\
 &  & RMSE & (1.48) & (0.41) & (0.29) & (0.28) & (0.24) &  & (2.31) & (0.99) & (0.76) & (0.63) & (0.5) \\
 & T & Bias & 0.51 & 0.82 & 0.34 & 0.26 & 0.1 &  & -1.6 & -1.74 & -0.6 & -0.63 & -0.22 \\
 &  & RMSE & (2.56) & (1.97) & (1.16) & (0.66) & (0.24) &  & (2.82) & (2.97) & (1.34) & (1.44) & (0.61) \\
 & U & Bias & 0.33 & 0.12 & 0.09 & 0.12 & 0.08 &  & -1.4 & -0.58 & -0.48 & -0.36 & -0.24 \\
 &  & RMSE & (1.49) & (0.38) & (0.28) & (0.27) & (0.22) &  & (2.32) & (0.98) & (0.75) & (0.64) & (0.47) \\
 & Non & Bias & 0.51 & 0.84 & 0.34 & 0.26 & 0.09 &  & -1.6 & -1.72 & -0.6 & -0.64 & -0.21 \\
 &  & RMSE & (2.56) & (1.98) & (1.16) & (0.66) & (0.24) &  & (2.82) & (2.98) & (1.34) & (1.45) & (0.64) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
0.5 & unmatched & Mean Num & 7.56 & 14.91 & 22.16 & 36.14 & 72.03 & -3.0 & 7.56 & 14.91 & 22.16 & 36.14 & 72.03 \\
 & U,T & Bias & -0.08 & 0.19 & 0.11 & 0.08 & 0.09 &  & -1.77 & -0.94 & -0.62 & -0.43 & -0.37 \\
 &  & RMSE & (2.03) & (0.51) & (0.35) & (0.29) & (0.2) &  & (2.73) & (1.72) & (1.26) & (0.82) & (0.64) \\
 & T & Bias & -0.05 & 0.65 & 0.14 & 0.3 & 0.21 &  & -0.13 & -0.57 & -1.01 & -0.75 & -0.81 \\
 &  & RMSE & (4.43) & (1.97) & (1.6) & (0.79) & (0.47) &  & (4.29) & (2.4) & (2.52) & (1.95) & (1.69) \\
 & U & Bias & -0.09 & 0.17 & 0.09 & 0.06 & 0.08 &  & -1.79 & -0.93 & -0.59 & -0.42 & -0.39 \\
 &  & RMSE & (2.04) & (0.51) & (0.32) & (0.27) & (0.2) &  & (2.73) & (1.71) & (1.22) & (0.82) & (0.63) \\
 & Non & Bias & 0.06 & 0.73 & 0.2 & 0.31 & 0.21 &  & -0.27 & -0.62 & -1.07 & -0.76 & -0.8 \\
 &  & RMSE & (4.47) & (2.19) & (1.6) & (0.79) & (0.48) &  & (4.23) & (2.41) & (2.52) & (1.94) & (1.69) \\
 &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_with_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.01 & 0.0 & 0.01 & 0.01 \\
 & U,T & Bias & 0.96 & 0.37 & 0.31 & 0.15 & 0.0 \\
 &  & RMSE & (2.45) & (1.4) & (0.81) & (0.51) & (0.32) \\
 & T & Bias & 0.98 & 0.37 & 0.29 & 0.15 & -0.0 \\
 &  & RMSE & (2.46) & (1.4) & (0.81) & (0.52) & (0.33) \\
 & U & Bias & 1.01 & 0.38 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.48) & (1.4) & (0.81) & (0.52) & (0.34) \\
 & Non & Bias & 1.02 & 0.38 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.47) & (1.4) & (0.81) & (0.52) & (0.34) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.15 & 0.11 & 0.12 & 0.13 & 0.14 \\
 & U,T & Bias & -0.08 & 0.04 & -0.02 & 0.02 & -0.01 \\
 &  & RMSE & (1.65) & (0.17) & (0.17) & (0.12) & (0.06) \\
 & T & Bias & -0.06 & 0.05 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.17) & (0.17) & (0.12) & (0.07) \\
 & U & Bias & -0.06 & 0.05 & -0.01 & 0.02 & -0.0 \\
 &  & RMSE & (1.66) & (0.17) & (0.18) & (0.12) & (0.07) \\
 & Non & Bias & -0.05 & 0.04 & -0.01 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.17) & (0.18) & (0.12) & (0.07) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 3.88 & 7.05 & 10.16 & 16.89 & 32.3 \\
 & U,T & Bias & -0.29 & -0.12 & -0.03 & -0.05 & -0.01 \\
 &  & RMSE & (0.9) & (0.35) & (0.21) & (0.19) & (0.16) \\
 & T & Bias & -0.26 & -0.42 & -0.18 & -0.12 & 0.0 \\
 &  & RMSE & (0.91) & (1.52) & (0.93) & (0.38) & (0.18) \\
 & U & Bias & -0.29 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.9) & (0.32) & (0.21) & (0.18) & (0.1) \\
 & Non & Bias & -0.25 & -0.42 & -0.19 & -0.11 & -0.0 \\
 &  & RMSE & (0.91) & (1.52) & (0.93) & (0.37) & (0.18) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.28 & 14.22 & 21.4 & 35.19 & 68.75 \\
 & U,T & Bias & -0.72 & -0.2 & -0.2 & -0.06 & 0.01 \\
 &  & RMSE & (1.34) & (0.58) & (0.53) & (0.29) & (0.26) \\
 & T & Bias & -0.73 & -0.04 & -0.37 & -0.55 & -0.1 \\
 &  & RMSE & (2.33) & (0.61) & (1.25) & (1.69) & (0.78) \\
 & U & Bias & -0.81 & -0.21 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.53) & (0.61) & (0.54) & (0.28) & (0.18) \\
 & Non & Bias & -0.72 & -0.05 & -0.37 & -0.57 & -0.12 \\
 &  & RMSE & (2.33) & (0.67) & (1.25) & (1.7) & (0.79) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.69 & 16.8 & 25.47 & 42.15 & 83.4 \\
 & U,T & Bias & -1.66 & -1.04 & -0.53 & -0.13 & -0.09 \\
 &  & RMSE & (2.64) & (1.97) & (1.36) & (0.55) & (0.46) \\
 & T & Bias & 0.03 & -0.18 & 0.45 & -0.58 & -0.13 \\
 &  & RMSE & (4.37) & (3.4) & (2.94) & (2.26) & (0.33) \\
 & U & Bias & -1.7 & -1.08 & -0.6 & -0.16 & -0.12 \\
 &  & RMSE & (2.68) & (2.03) & (1.4) & (0.55) & (0.38) \\
 & Non & Bias & 0.03 & -0.18 & 0.44 & -0.58 & -0.11 \\
 &  & RMSE & (4.37) & (3.4) & (2.95) & (2.26) & (0.35) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_with_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.01 & 0.0 & 0.01 & 0.02 \\
 & U,T & Bias & 1.11 & 0.53 & 0.31 & 0.14 & 0.0 \\
 &  & RMSE & (2.62) & (1.68) & (0.8) & (0.51) & (0.32) \\
 & T & Bias & 1.09 & 0.57 & 0.29 & 0.15 & -0.0 \\
 &  & RMSE & (2.62) & (1.73) & (0.81) & (0.52) & (0.33) \\
 & U & Bias & 1.12 & 0.56 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.63) & (1.72) & (0.81) & (0.52) & (0.34) \\
 & Non & Bias & 1.12 & 0.58 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (2.63) & (1.73) & (0.81) & (0.52) & (0.34) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.19 & 0.1 & 0.12 & 0.11 & 0.16 \\
 & U,T & Bias & -0.04 & 0.08 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.46) & (0.17) & (0.12) & (0.06) \\
 & T & Bias & -0.04 & 0.06 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & U & Bias & -0.04 & 0.06 & -0.01 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & Non & Bias & -0.04 & 0.06 & -0.01 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.46) & (0.18) & (0.12) & (0.07) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 3.68 & 7.0 & 10.18 & 17.07 & 32.25 \\
 & U,T & Bias & -0.29 & -0.12 & -0.02 & -0.05 & -0.01 \\
 &  & RMSE & (0.9) & (0.35) & (0.21) & (0.19) & (0.17) \\
 & T & Bias & -0.82 & -0.3 & -0.08 & -0.11 & 0.0 \\
 &  & RMSE & (2.14) & (1.09) & (0.44) & (0.37) & (0.18) \\
 & U & Bias & -0.29 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.9) & (0.32) & (0.21) & (0.18) & (0.1) \\
 & Non & Bias & -0.81 & -0.29 & -0.09 & -0.11 & -0.0 \\
 &  & RMSE & (2.14) & (1.09) & (0.44) & (0.37) & (0.18) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.41 & 14.09 & 21.06 & 34.86 & 68.49 \\
 & U,T & Bias & -0.69 & -0.2 & -0.19 & -0.05 & 0.01 \\
 &  & RMSE & (1.28) & (0.58) & (0.53) & (0.29) & (0.26) \\
 & T & Bias & -0.7 & -0.03 & -0.17 & -0.06 & -0.12 \\
 &  & RMSE & (2.3) & (0.61) & (0.52) & (0.35) & (0.62) \\
 & U & Bias & -0.78 & -0.21 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.49) & (0.61) & (0.54) & (0.28) & (0.18) \\
 & Non & Bias & -0.7 & -0.05 & -0.18 & -0.05 & -0.13 \\
 &  & RMSE & (2.3) & (0.67) & (0.53) & (0.35) & (0.63) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.76 & 16.78 & 25.26 & 42.16 & 83.29 \\
 & U,T & Bias & -1.66 & -1.03 & -0.52 & -0.13 & -0.08 \\
 &  & RMSE & (2.64) & (1.97) & (1.36) & (0.55) & (0.46) \\
 & T & Bias & 0.0 & 0.3 & 0.29 & -0.29 & -0.17 \\
 &  & RMSE & (4.2) & (3.33) & (2.89) & (1.29) & (0.72) \\
 & U & Bias & -1.7 & -1.08 & -0.6 & -0.16 & -0.12 \\
 &  & RMSE & (2.68) & (2.03) & (1.4) & (0.55) & (0.38) \\
 & Non & Bias & 0.0 & 0.27 & 0.22 & -0.3 & -0.15 \\
 &  & RMSE & (4.2) & (3.36) & (2.94) & (1.29) & (0.73) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_without_dummy_with_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.01 & 0.0 & 0.0 & 0.02 \\
 & U,T & Bias & 0.61 & 0.6 & 0.31 & 0.13 & -0.0 \\
 &  & RMSE & (1.78) & (1.77) & (0.8) & (0.5) & (0.32) \\
 & T & Bias & 0.57 & 0.61 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (1.75) & (1.81) & (0.81) & (0.52) & (0.33) \\
 & U & Bias & 0.59 & 0.64 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (1.76) & (1.82) & (0.81) & (0.52) & (0.34) \\
 & Non & Bias & 0.58 & 0.62 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (1.76) & (1.81) & (0.81) & (0.52) & (0.34) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.16 & 0.09 & 0.17 & 0.13 & 0.12 \\
 & U,T & Bias & -0.02 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.63) & (0.38) & (0.17) & (0.12) & (0.06) \\
 & T & Bias & -0.01 & 0.06 & -0.01 & 0.02 & -0.0 \\
 &  & RMSE & (1.63) & (0.38) & (0.18) & (0.12) & (0.07) \\
 & U & Bias & -0.02 & 0.06 & -0.01 & 0.02 & -0.0 \\
 &  & RMSE & (1.63) & (0.38) & (0.18) & (0.12) & (0.07) \\
 & Non & Bias & -0.02 & 0.06 & -0.01 & 0.02 & -0.0 \\
 &  & RMSE & (1.63) & (0.38) & (0.18) & (0.12) & (0.07) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 3.81 & 7.05 & 9.82 & 16.89 & 31.83 \\
 & U,T & Bias & -0.29 & -0.12 & -0.02 & -0.05 & -0.01 \\
 &  & RMSE & (0.9) & (0.35) & (0.2) & (0.19) & (0.17) \\
 & T & Bias & -0.52 & -0.19 & -0.22 & -0.12 & 0.0 \\
 &  & RMSE & (1.51) & (0.89) & (0.98) & (0.38) & (0.18) \\
 & U & Bias & -0.29 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.9) & (0.32) & (0.21) & (0.18) & (0.1) \\
 & Non & Bias & -0.52 & -0.19 & -0.22 & -0.1 & -0.0 \\
 &  & RMSE & (1.51) & (0.89) & (0.98) & (0.37) & (0.18) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.24 & 13.85 & 21.25 & 34.97 & 69.07 \\
 & U,T & Bias & -0.71 & -0.2 & -0.19 & -0.05 & 0.02 \\
 &  & RMSE & (1.34) & (0.58) & (0.53) & (0.29) & (0.26) \\
 & T & Bias & -0.9 & -0.16 & -0.17 & -0.08 & -0.14 \\
 &  & RMSE & (3.44) & (0.97) & (0.52) & (0.28) & (0.79) \\
 & U & Bias & -0.81 & -0.21 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.53) & (0.61) & (0.54) & (0.28) & (0.18) \\
 & Non & Bias & -0.9 & -0.14 & -0.23 & -0.07 & -0.15 \\
 &  & RMSE & (3.44) & (0.97) & (0.83) & (0.28) & (0.8) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.57 & 16.8 & 25.67 & 42.29 & 83.12 \\
 & U,T & Bias & -1.66 & -1.02 & -0.52 & -0.13 & -0.08 \\
 &  & RMSE & (2.64) & (1.97) & (1.36) & (0.55) & (0.46) \\
 & T & Bias & -0.09 & 0.16 & 0.33 & -0.57 & -0.16 \\
 &  & RMSE & (4.55) & (3.36) & (2.81) & (1.89) & (1.02) \\
 & U & Bias & -1.7 & -1.08 & -0.6 & -0.16 & -0.12 \\
 &  & RMSE & (2.68) & (2.03) & (1.4) & (0.55) & (0.38) \\
 & Non & Bias & -0.23 & 0.1 & 0.29 & -0.58 & -0.14 \\
 &  & RMSE & (4.37) & (3.41) & (2.84) & (1.89) & (1.03) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}


==> figuretable/estimation_results_single_market_without_dummy_without_IR.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lc|cccccc}
\toprule 
 & Num of agents &  & 10 & 20 & 30 & 50 & 100 \\
$\beta$ &  &  &  &  &  &  &  \\
\midrule 
1.0 & unmatched & Mean Num & 0.0 & 0.01 & 0.0 & 0.01 & 0.01 \\
 & U,T & Bias & 0.61 & 0.6 & 0.31 & 0.13 & -0.0 \\
 &  & RMSE & (1.76) & (1.77) & (0.8) & (0.49) & (0.32) \\
 & T & Bias & 0.57 & 0.61 & 0.3 & 0.14 & -0.01 \\
 &  & RMSE & (1.76) & (1.81) & (0.81) & (0.52) & (0.33) \\
 & U & Bias & 0.61 & 0.64 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (1.76) & (1.82) & (0.81) & (0.52) & (0.34) \\
 & Non & Bias & 0.61 & 0.64 & 0.29 & 0.15 & -0.01 \\
 &  & RMSE & (1.76) & (1.82) & (0.81) & (0.52) & (0.34) \\
 &  &  &  &  &  &  &  \\
0.0 & unmatched & Mean Num & 0.2 & 0.14 & 0.16 & 0.11 & 0.16 \\
 & U,T & Bias & -0.05 & 0.09 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.64) & (0.46) & (0.17) & (0.12) & (0.06) \\
 & T & Bias & -0.04 & 0.08 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & U & Bias & -0.04 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.46) & (0.18) & (0.12) & (0.07) \\
 & Non & Bias & -0.05 & 0.07 & -0.02 & 0.02 & -0.0 \\
 &  & RMSE & (1.65) & (0.46) & (0.18) & (0.12) & (0.07) \\
 &  &  &  &  &  &  &  \\
-1.0 & unmatched & Mean Num & 3.65 & 6.96 & 10.32 & 16.62 & 31.89 \\
 & U,T & Bias & -0.29 & -0.12 & -0.02 & -0.05 & -0.01 \\
 &  & RMSE & (0.9) & (0.34) & (0.21) & (0.19) & (0.17) \\
 & T & Bias & -0.28 & -0.39 & -0.22 & -0.12 & 0.0 \\
 &  & RMSE & (0.92) & (1.52) & (0.98) & (0.38) & (0.18) \\
 & U & Bias & -0.29 & -0.11 & -0.04 & -0.04 & -0.0 \\
 &  & RMSE & (0.9) & (0.32) & (0.21) & (0.18) & (0.1) \\
 & Non & Bias & -0.26 & -0.39 & -0.22 & -0.11 & -0.0 \\
 &  & RMSE & (0.94) & (1.52) & (0.98) & (0.37) & (0.18) \\
 &  &  &  &  &  &  &  \\
-2.0 & unmatched & Mean Num & 7.46 & 14.06 & 21.21 & 35.01 & 68.58 \\
 & U,T & Bias & -0.69 & -0.2 & -0.18 & -0.04 & 0.03 \\
 &  & RMSE & (1.33) & (0.58) & (0.53) & (0.29) & (0.27) \\
 & T & Bias & -0.71 & -0.04 & -1.04 & -0.34 & -0.14 \\
 &  & RMSE & (2.31) & (0.61) & (2.36) & (1.26) & (0.77) \\
 & U & Bias & -0.81 & -0.21 & -0.22 & -0.09 & -0.01 \\
 &  & RMSE & (1.53) & (0.61) & (0.54) & (0.28) & (0.18) \\
 & Non & Bias & -0.71 & -0.02 & -1.04 & -0.33 & -0.16 \\
 &  & RMSE & (2.31) & (0.62) & (2.36) & (1.26) & (0.78) \\
 &  &  &  &  &  &  &  \\
-3.0 & unmatched & Mean Num & 8.47 & 16.88 & 25.39 & 42.02 & 83.34 \\
 & U,T & Bias & -1.65 & -0.91 & -0.47 & -0.11 & -0.06 \\
 &  & RMSE & (2.64) & (1.81) & (1.23) & (0.54) & (0.47) \\
 & T & Bias & -0.11 & 0.15 & -0.3 & -0.23 & -0.15 \\
 &  & RMSE & (4.44) & (3.18) & (3.66) & (1.28) & (0.74) \\
 & U & Bias & -1.7 & -1.08 & -0.6 & -0.16 & -0.12 \\
 &  & RMSE & (2.68) & (2.03) & (1.4) & (0.55) & (0.38) \\
 & Non & Bias & -0.11 & 0.11 & -0.31 & -0.26 & -0.13 \\
 &  & RMSE & (4.44) & (3.21) & (3.67) & (1.29) & (0.74) \\
 &  &  &  &  &  &  &  \\
\hline 
\bottomrule 
\end{tabular}

